Do ImageNet Classifiers Generalize to ImageNet?

We build new test sets for the CIFAR-10 and ImageNet datasets. Both benchmarks have been the focus of intense research for almost a decade, raising the danger of overfitting to excessively re-used test sets. By closely following the original dataset creation processes, we test to what extent current classification models generalize to new data. We evaluate a broad range of models and find accuracy drops of 3% - 15% on CIFAR-10 and 11% - 14% on ImageNet. However, accuracy gains on the original test sets translate to larger gains on the new test sets. Our results suggest that the accuracy drops are not caused by adaptivity, but by the models' inability to generalize to slightly "harder" images than those found in the original test sets.

==> tables/imagenetv2-a-44_top1_model_results_table.tex <==
\begin{tabular}{rp{4.75cm}rrrrr}
\toprule 
\multicolumn{7}{c}{\textbf{ImageNet Top-1 \dataseta}} \\ 
\midrule
\multicolumn{1}{l}{Orig.} &                               &                                        &                                          &   & \multicolumn{1}{l}{New} &  \\ 
 \multicolumn{1}{l}{Rank} & Model & Orig. Accuracy & New Accuracy & Gap & \multicolumn{1}{l}{Rank} & $\Delta$ Rank \\
\midrule
 1 &  \model{pnasnet\_large\_tf} &  82.9 {\footnotesize \textcolor{gray}{[82.5, 83.2]}} &  80.2 {\footnotesize \textcolor{gray}{[79.4, 80.9]}} &  2.7 &  2 &  -1 \\
 2 &  \model{pnasnet5large} &  82.7 {\footnotesize \textcolor{gray}{[82.4, 83.1]}} &  80.3 {\footnotesize \textcolor{gray}{[79.5, 81.1]}} &  2.4 &  1 &  1 \\
 3 &  \model{nasnet\_large\_tf} &  82.7 {\footnotesize \textcolor{gray}{[82.4, 83.0]}} &  80.1 {\footnotesize \textcolor{gray}{[79.3, 80.9]}} &  2.6 &  3 &  0 \\
 4 &  \model{nasnetalarge} &  82.5 {\footnotesize \textcolor{gray}{[82.2, 82.8]}} &  80.0 {\footnotesize \textcolor{gray}{[79.2, 80.8]}} &  2.5 &  4 &  0 \\
 5 &  \model{senet154} &  81.3 {\footnotesize \textcolor{gray}{[81.0, 81.6]}} &  78.7 {\footnotesize \textcolor{gray}{[77.8, 79.5]}} &  2.6 &  5 &  0 \\
 6 &  \model{polynet} &  80.9 {\footnotesize \textcolor{gray}{[80.5, 81.2]}} &  78.5 {\footnotesize \textcolor{gray}{[77.7, 79.3]}} &  2.3 &  6 &  0 \\
 7 &  \model{inception\_resnet\_v2\_tf} &  80.4 {\footnotesize \textcolor{gray}{[80.0, 80.7]}} &  77.9 {\footnotesize \textcolor{gray}{[77.1, 78.7]}} &  2.5 &  8 &  -1 \\
 8 &  \model{inceptionresnetv2} &  80.3 {\footnotesize \textcolor{gray}{[79.9, 80.6]}} &  78.0 {\footnotesize \textcolor{gray}{[77.2, 78.8]}} &  2.3 &  7 &  1 \\
 9 &  \model{se\_resnext101\_32x4d} &  80.2 {\footnotesize \textcolor{gray}{[79.9, 80.6]}} &  77.6 {\footnotesize \textcolor{gray}{[76.8, 78.5]}} &  2.6 &  11 &  -2 \\
 10 &  \model{inception\_v4\_tf} &  80.2 {\footnotesize \textcolor{gray}{[79.8, 80.5]}} &  77.8 {\footnotesize \textcolor{gray}{[77.0, 78.6]}} &  2.4 &  10 &  0 \\
 11 &  \model{inceptionv4} &  80.1 {\footnotesize \textcolor{gray}{[79.7, 80.4]}} &  77.9 {\footnotesize \textcolor{gray}{[77.0, 78.7]}} &  2.2 &  9 &  2 \\
 12 &  \model{dpn107} &  79.7 {\footnotesize \textcolor{gray}{[79.4, 80.1]}} &  76.6 {\footnotesize \textcolor{gray}{[75.8, 77.5]}} &  3.1 &  12 &  0 \\
 13 &  \model{dpn131} &  79.4 {\footnotesize \textcolor{gray}{[79.1, 79.8]}} &  76.6 {\footnotesize \textcolor{gray}{[75.7, 77.4]}} &  2.9 &  13 &  0 \\
 14 &  \model{dpn92} &  79.4 {\footnotesize \textcolor{gray}{[79.0, 79.8]}} &  76.3 {\footnotesize \textcolor{gray}{[75.5, 77.1]}} &  3.1 &  17 &  -3 \\
 15 &  \model{dpn98} &  79.2 {\footnotesize \textcolor{gray}{[78.9, 79.6]}} &  76.3 {\footnotesize \textcolor{gray}{[75.5, 77.2]}} &  2.9 &  16 &  -1 \\
 16 &  \model{se\_resnext50\_32x4d} &  79.1 {\footnotesize \textcolor{gray}{[78.7, 79.4]}} &  76.5 {\footnotesize \textcolor{gray}{[75.7, 77.3]}} &  2.6 &  14 &  2 \\
 17 &  \model{resnext101\_64x4d} &  79.0 {\footnotesize \textcolor{gray}{[78.6, 79.3]}} &  75.6 {\footnotesize \textcolor{gray}{[74.7, 76.4]}} &  3.4 &  20 &  -3 \\
 18 &  \model{xception} &  78.8 {\footnotesize \textcolor{gray}{[78.5, 79.2]}} &  76.4 {\footnotesize \textcolor{gray}{[75.5, 77.2]}} &  2.5 &  15 &  3 \\
 19 &  \model{se\_resnet152} &  78.7 {\footnotesize \textcolor{gray}{[78.3, 79.0]}} &  76.1 {\footnotesize \textcolor{gray}{[75.3, 76.9]}} &  2.5 &  18 &  1 \\
 20 &  \model{se\_resnet101} &  78.4 {\footnotesize \textcolor{gray}{[78.0, 78.8]}} &  75.8 {\footnotesize \textcolor{gray}{[75.0, 76.7]}} &  2.6 &  19 &  1 \\
 21 &  \model{resnet152} &  78.3 {\footnotesize \textcolor{gray}{[77.9, 78.7]}} &  75.3 {\footnotesize \textcolor{gray}{[74.5, 76.2]}} &  3.0 &  22 &  -1 \\
 22 &  \model{resnext101\_32x4d} &  78.2 {\footnotesize \textcolor{gray}{[77.8, 78.5]}} &  75.4 {\footnotesize \textcolor{gray}{[74.5, 76.2]}} &  2.8 &  21 &  1 \\
 23 &  \model{inception\_v3\_tf} &  78.0 {\footnotesize \textcolor{gray}{[77.6, 78.3]}} &  75.0 {\footnotesize \textcolor{gray}{[74.2, 75.9]}} &  2.9 &  24 &  -1 \\
 24 &  \model{resnet\_v2\_152\_tf} &  77.8 {\footnotesize \textcolor{gray}{[77.4, 78.1]}} &  75.2 {\footnotesize \textcolor{gray}{[74.4, 76.1]}} &  2.6 &  23 &  1 \\
 25 &  \model{se\_resnet50} &  77.6 {\footnotesize \textcolor{gray}{[77.3, 78.0]}} &  74.2 {\footnotesize \textcolor{gray}{[73.3, 75.1]}} &  3.4 &  30 &  -5 \\
 26 &  \model{fbresnet152} &  77.4 {\footnotesize \textcolor{gray}{[77.0, 77.8]}} &  74.8 {\footnotesize \textcolor{gray}{[74.0, 75.7]}} &  2.6 &  25 &  1 \\
 27 &  \model{resnet101} &  77.4 {\footnotesize \textcolor{gray}{[77.0, 77.7]}} &  74.5 {\footnotesize \textcolor{gray}{[73.6, 75.3]}} &  2.9 &  29 &  -2 \\
 28 &  \model{inceptionv3} &  77.3 {\footnotesize \textcolor{gray}{[77.0, 77.7]}} &  74.5 {\footnotesize \textcolor{gray}{[73.6, 75.4]}} &  2.8 &  28 &  0 \\
 29 &  \model{inception\_v3} &  77.2 {\footnotesize \textcolor{gray}{[76.8, 77.6]}} &  74.7 {\footnotesize \textcolor{gray}{[73.8, 75.6]}} &  2.5 &  26 &  3 \\
 30 &  \model{densenet161} &  77.1 {\footnotesize \textcolor{gray}{[76.8, 77.5]}} &  74.6 {\footnotesize \textcolor{gray}{[73.7, 75.4]}} &  2.6 &  27 &  3 \\
 31 &  \model{dpn68b} &  77.0 {\footnotesize \textcolor{gray}{[76.7, 77.4]}} &  73.8 {\footnotesize \textcolor{gray}{[72.9, 74.7]}} &  3.2 &  33 &  -2 \\
 32 &  \model{resnet\_v2\_101\_tf} &  77.0 {\footnotesize \textcolor{gray}{[76.6, 77.3]}} &  74.0 {\footnotesize \textcolor{gray}{[73.1, 74.8]}} &  3.0 &  31 &  1 \\
 33 &  \model{densenet201} &  76.9 {\footnotesize \textcolor{gray}{[76.5, 77.3]}} &  73.9 {\footnotesize \textcolor{gray}{[73.1, 74.8]}} &  3.0 &  32 &  1 \\
 34 &  \model{resnet\_v1\_152\_tf} &  76.8 {\footnotesize \textcolor{gray}{[76.4, 77.2]}} &  73.7 {\footnotesize \textcolor{gray}{[72.9, 74.6]}} &  3.1 &  34 &  0 \\
 35 &  \model{resnet\_v1\_101\_tf} &  76.4 {\footnotesize \textcolor{gray}{[76.0, 76.8]}} &  73.4 {\footnotesize \textcolor{gray}{[72.5, 74.2]}} &  3.0 &  35 &  0 \\
 36 &  \model{cafferesnet101} &  76.2 {\footnotesize \textcolor{gray}{[75.8, 76.6]}} &  72.9 {\footnotesize \textcolor{gray}{[72.0, 73.7]}} &  3.3 &  37 &  -1 \\
 37 &  \model{resnet50} &  76.1 {\footnotesize \textcolor{gray}{[75.8, 76.5]}} &  72.7 {\footnotesize \textcolor{gray}{[71.8, 73.6]}} &  3.4 &  38 &  -1 \\
 38 &  \model{dpn68} &  75.9 {\footnotesize \textcolor{gray}{[75.5, 76.2]}} &  73.0 {\footnotesize \textcolor{gray}{[72.1, 73.8]}} &  2.9 &  36 &  2 \\
 39 &  \model{densenet169} &  75.6 {\footnotesize \textcolor{gray}{[75.2, 76.0]}} &  72.3 {\footnotesize \textcolor{gray}{[71.4, 73.1]}} &  3.3 &  40 &  -1 \\
 40 &  \model{resnet\_v2\_50\_tf} &  75.6 {\footnotesize \textcolor{gray}{[75.2, 76.0]}} &  72.3 {\footnotesize \textcolor{gray}{[71.4, 73.2]}} &  3.3 &  39 &  1 \\
 41 &  \model{resnet\_v1\_50\_tf} &  75.2 {\footnotesize \textcolor{gray}{[74.8, 75.6]}} &  71.9 {\footnotesize \textcolor{gray}{[71.0, 72.8]}} &  3.3 &  41 &  0 \\
 42 &  \model{densenet121} &  74.4 {\footnotesize \textcolor{gray}{[74.0, 74.8]}} &  70.5 {\footnotesize \textcolor{gray}{[69.6, 71.4]}} &  3.9 &  47 &  -5 \\
 43 &  \model{vgg19\_bn} &  74.2 {\footnotesize \textcolor{gray}{[73.8, 74.6]}} &  71.4 {\footnotesize \textcolor{gray}{[70.5, 72.3]}} &  2.8 &  42 &  1 \\
 44 &  \model{pnasnet\_mobile\_tf} &  74.1 {\footnotesize \textcolor{gray}{[73.8, 74.5]}} &  70.6 {\footnotesize \textcolor{gray}{[69.7, 71.5]}} &  3.6 &  46 &  -2 \\
 45 &  \model{nasnetamobile} &  74.1 {\footnotesize \textcolor{gray}{[73.7, 74.5]}} &  70.9 {\footnotesize \textcolor{gray}{[70.0, 71.8]}} &  3.2 &  45 &  0 \\
 46 &  \model{inception\_v2\_tf} &  74.0 {\footnotesize \textcolor{gray}{[73.6, 74.4]}} &  71.1 {\footnotesize \textcolor{gray}{[70.2, 72.0]}} &  2.9 &  44 &  2 \\
 47 &  \model{nasnet\_mobile\_tf} &  74.0 {\footnotesize \textcolor{gray}{[73.6, 74.4]}} &  70.0 {\footnotesize \textcolor{gray}{[69.0, 70.8]}} &  4.0 &  50 &  -3 \\
 48 &  \model{bninception} &  73.5 {\footnotesize \textcolor{gray}{[73.1, 73.9]}} &  71.3 {\footnotesize \textcolor{gray}{[70.4, 72.2]}} &  2.2 &  43 &  5 \\
 49 &  \model{vgg16\_bn} &  73.4 {\footnotesize \textcolor{gray}{[73.0, 73.7]}} &  70.2 {\footnotesize \textcolor{gray}{[69.3, 71.1]}} &  3.1 &  48 &  1 \\
 50 &  \model{resnet34} &  73.3 {\footnotesize \textcolor{gray}{[72.9, 73.7]}} &  70.2 {\footnotesize \textcolor{gray}{[69.2, 71.0]}} &  3.2 &  49 &  1 \\
 51 &  \model{vgg19} &  72.4 {\footnotesize \textcolor{gray}{[72.0, 72.8]}} &  68.7 {\footnotesize \textcolor{gray}{[67.8, 69.6]}} &  3.7 &  51 &  0 \\
 52 &  \model{vgg16} &  71.6 {\footnotesize \textcolor{gray}{[71.2, 72.0]}} &  68.0 {\footnotesize \textcolor{gray}{[67.0, 68.9]}} &  3.6 &  52 &  0 \\
 53 &  \model{vgg13\_bn} &  71.6 {\footnotesize \textcolor{gray}{[71.2, 72.0]}} &  67.3 {\footnotesize \textcolor{gray}{[66.4, 68.2]}} &  4.3 &  55 &  -2 \\
 54 &  \model{mobilenet\_v1\_tf} &  71.0 {\footnotesize \textcolor{gray}{[70.6, 71.4]}} &  66.1 {\footnotesize \textcolor{gray}{[65.2, 67.0]}} &  4.9 &  59 &  -5 \\
 55 &  \model{vgg\_19\_tf} &  71.0 {\footnotesize \textcolor{gray}{[70.6, 71.4]}} &  67.4 {\footnotesize \textcolor{gray}{[66.5, 68.3]}} &  3.6 &  54 &  1 \\
 56 &  \model{vgg\_16\_tf} &  70.9 {\footnotesize \textcolor{gray}{[70.5, 71.3]}} &  67.6 {\footnotesize \textcolor{gray}{[66.7, 68.5]}} &  3.3 &  53 &  3 \\
 57 &  \model{vgg11\_bn} &  70.4 {\footnotesize \textcolor{gray}{[70.0, 70.8]}} &  66.4 {\footnotesize \textcolor{gray}{[65.5, 67.3]}} &  4.0 &  58 &  -1 \\
 58 &  \model{vgg13} &  69.9 {\footnotesize \textcolor{gray}{[69.5, 70.3]}} &  66.0 {\footnotesize \textcolor{gray}{[65.0, 66.9]}} &  4.0 &  60 &  -2 \\
 59 &  \model{inception\_v1\_tf} &  69.8 {\footnotesize \textcolor{gray}{[69.4, 70.2]}} &  66.4 {\footnotesize \textcolor{gray}{[65.5, 67.4]}} &  3.3 &  57 &  2 \\
 60 &  \model{resnet18} &  69.8 {\footnotesize \textcolor{gray}{[69.4, 70.2]}} &  66.6 {\footnotesize \textcolor{gray}{[65.7, 67.5]}} &  3.2 &  56 &  4 \\
 61 &  \model{vgg11} &  69.0 {\footnotesize \textcolor{gray}{[68.6, 69.4]}} &  64.6 {\footnotesize \textcolor{gray}{[63.7, 65.6]}} &  4.4 &  61 &  0 \\
 62 &  \model{squeezenet1\_1} &  58.2 {\footnotesize \textcolor{gray}{[57.7, 58.6]}} &  54.4 {\footnotesize \textcolor{gray}{[53.4, 55.4]}} &  3.8 &  62 &  0 \\
 63 &  \model{squeezenet1\_0} &  58.1 {\footnotesize \textcolor{gray}{[57.7, 58.5]}} &  53.4 {\footnotesize \textcolor{gray}{[52.4, 54.4]}} &  4.7 &  63 &  0 \\
 64 &  \model{alexnet} &  56.5 {\footnotesize \textcolor{gray}{[56.1, 57.0]}} &  51.3 {\footnotesize \textcolor{gray}{[50.3, 52.3]}} &  5.2 &  64 &  0 \\
 65 &  \model{fv\_64k} &  35.1 {\footnotesize \textcolor{gray}{[34.7, 35.5]}} &  29.1 {\footnotesize \textcolor{gray}{[28.2, 30.0]}} &  6.0 &  65 &  0 \\
 66 &  \model{fv\_16k} &  28.3 {\footnotesize \textcolor{gray}{[27.9, 28.7]}} &  23.4 {\footnotesize \textcolor{gray}{[22.5, 24.2]}} &  5.0 &  66 &  0 \\
 67 &  \model{fv\_4k} &  21.2 {\footnotesize \textcolor{gray}{[20.8, 21.5]}} &  17.8 {\footnotesize \textcolor{gray}{[17.0, 18.5]}} &  3.4 &  67 &  0 \\
\bottomrule
\end{tabular}


==> tables/imagenetv2-a-44_top5_model_results_table.tex <==
\begin{tabular}{rp{4.75cm}rrrrr}
\toprule 
\multicolumn{7}{c}{\textbf{ImageNet Top-5 \dataseta}} \\ 
\midrule
\multicolumn{1}{l}{Orig.} &                               &                                        &                                          &   & \multicolumn{1}{l}{New} &  \\ 
 \multicolumn{1}{l}{Rank} & Model & Orig. Accuracy & New Accuracy & Gap & \multicolumn{1}{l}{Rank} & $\Delta$ Rank \\
\midrule
 1 &  \model{pnasnet\_large\_tf} &  96.2 {\footnotesize \textcolor{gray}{[96.0, 96.3]}} &  95.6 {\footnotesize \textcolor{gray}{[95.2, 96.0]}} &  0.6 &  2 &  -1 \\
 2 &  \model{nasnet\_large\_tf} &  96.2 {\footnotesize \textcolor{gray}{[96.0, 96.3]}} &  95.7 {\footnotesize \textcolor{gray}{[95.2, 96.0]}} &  0.5 &  1 &  1 \\
 3 &  \model{nasnetalarge} &  96.0 {\footnotesize \textcolor{gray}{[95.8, 96.2]}} &  95.3 {\footnotesize \textcolor{gray}{[94.9, 95.8]}} &  0.7 &  4 &  -1 \\
 4 &  \model{pnasnet5large} &  96.0 {\footnotesize \textcolor{gray}{[95.8, 96.2]}} &  95.5 {\footnotesize \textcolor{gray}{[95.0, 95.9]}} &  0.5 &  3 &  1 \\
 5 &  \model{polynet} &  95.6 {\footnotesize \textcolor{gray}{[95.4, 95.7]}} &  94.9 {\footnotesize \textcolor{gray}{[94.4, 95.3]}} &  0.7 &  5 &  0 \\
 6 &  \model{senet154} &  95.5 {\footnotesize \textcolor{gray}{[95.3, 95.7]}} &  94.8 {\footnotesize \textcolor{gray}{[94.3, 95.2]}} &  0.7 &  6 &  0 \\
 7 &  \model{inception\_resnet\_v2\_tf} &  95.2 {\footnotesize \textcolor{gray}{[95.1, 95.4]}} &  94.7 {\footnotesize \textcolor{gray}{[94.2, 95.1]}} &  0.6 &  7 &  0 \\
 8 &  \model{inception\_v4\_tf} &  95.2 {\footnotesize \textcolor{gray}{[95.0, 95.4]}} &  94.4 {\footnotesize \textcolor{gray}{[94.0, 94.9]}} &  0.8 &  9 &  -1 \\
 9 &  \model{inceptionresnetv2} &  95.1 {\footnotesize \textcolor{gray}{[94.9, 95.3]}} &  94.5 {\footnotesize \textcolor{gray}{[94.1, 95.0]}} &  0.6 &  8 &  1 \\
 10 &  \model{se\_resnext101\_32x4d} &  95.0 {\footnotesize \textcolor{gray}{[94.8, 95.2]}} &  94.3 {\footnotesize \textcolor{gray}{[93.8, 94.7]}} &  0.7 &  11 &  -1 \\
 11 &  \model{inceptionv4} &  94.9 {\footnotesize \textcolor{gray}{[94.7, 95.1]}} &  94.3 {\footnotesize \textcolor{gray}{[93.8, 94.7]}} &  0.6 &  10 &  1 \\
 12 &  \model{dpn107} &  94.7 {\footnotesize \textcolor{gray}{[94.5, 94.9]}} &  93.7 {\footnotesize \textcolor{gray}{[93.2, 94.2]}} &  1.0 &  12 &  0 \\
 13 &  \model{dpn92} &  94.6 {\footnotesize \textcolor{gray}{[94.4, 94.8]}} &  93.7 {\footnotesize \textcolor{gray}{[93.2, 94.2]}} &  0.9 &  14 &  -1 \\
 14 &  \model{dpn131} &  94.6 {\footnotesize \textcolor{gray}{[94.4, 94.8]}} &  93.5 {\footnotesize \textcolor{gray}{[92.9, 93.9]}} &  1.1 &  20 &  -6 \\
 15 &  \model{dpn98} &  94.5 {\footnotesize \textcolor{gray}{[94.3, 94.7]}} &  93.6 {\footnotesize \textcolor{gray}{[93.1, 94.1]}} &  0.9 &  17 &  -2 \\
 16 &  \model{se\_resnext50\_32x4d} &  94.4 {\footnotesize \textcolor{gray}{[94.2, 94.6]}} &  93.6 {\footnotesize \textcolor{gray}{[93.1, 94.1]}} &  0.8 &  16 &  0 \\
 17 &  \model{se\_resnet152} &  94.4 {\footnotesize \textcolor{gray}{[94.2, 94.6]}} &  93.7 {\footnotesize \textcolor{gray}{[93.2, 94.2]}} &  0.7 &  13 &  4 \\
 18 &  \model{xception} &  94.3 {\footnotesize \textcolor{gray}{[94.1, 94.5]}} &  93.6 {\footnotesize \textcolor{gray}{[93.1, 94.1]}} &  0.7 &  18 &  0 \\
 19 &  \model{se\_resnet101} &  94.3 {\footnotesize \textcolor{gray}{[94.1, 94.5]}} &  93.6 {\footnotesize \textcolor{gray}{[93.1, 94.0]}} &  0.7 &  19 &  0 \\
 20 &  \model{resnext101\_64x4d} &  94.3 {\footnotesize \textcolor{gray}{[94.0, 94.5]}} &  93.3 {\footnotesize \textcolor{gray}{[92.8, 93.8]}} &  0.9 &  22 &  -2 \\
 21 &  \model{resnet\_v2\_152\_tf} &  94.1 {\footnotesize \textcolor{gray}{[93.9, 94.3]}} &  93.4 {\footnotesize \textcolor{gray}{[92.9, 93.9]}} &  0.7 &  21 &  0 \\
 22 &  \model{resnet152} &  94.0 {\footnotesize \textcolor{gray}{[93.8, 94.3]}} &  93.7 {\footnotesize \textcolor{gray}{[93.2, 94.2]}} &  0.4 &  15 &  7 \\
 23 &  \model{inception\_v3\_tf} &  93.9 {\footnotesize \textcolor{gray}{[93.7, 94.1]}} &  92.8 {\footnotesize \textcolor{gray}{[92.3, 93.3]}} &  1.1 &  25 &  -2 \\
 24 &  \model{resnext101\_32x4d} &  93.9 {\footnotesize \textcolor{gray}{[93.7, 94.1]}} &  92.7 {\footnotesize \textcolor{gray}{[92.2, 93.2]}} &  1.2 &  28 &  -4 \\
 25 &  \model{se\_resnet50} &  93.8 {\footnotesize \textcolor{gray}{[93.5, 94.0]}} &  93.0 {\footnotesize \textcolor{gray}{[92.4, 93.5]}} &  0.8 &  24 &  1 \\
 26 &  \model{resnet\_v2\_101\_tf} &  93.7 {\footnotesize \textcolor{gray}{[93.5, 93.9]}} &  93.2 {\footnotesize \textcolor{gray}{[92.7, 93.7]}} &  0.5 &  23 &  3 \\
 27 &  \model{fbresnet152} &  93.6 {\footnotesize \textcolor{gray}{[93.4, 93.8]}} &  92.7 {\footnotesize \textcolor{gray}{[92.1, 93.2]}} &  0.9 &  29 &  -2 \\
 28 &  \model{dpn68b} &  93.6 {\footnotesize \textcolor{gray}{[93.4, 93.8]}} &  92.7 {\footnotesize \textcolor{gray}{[92.1, 93.2]}} &  0.9 &  31 &  -3 \\
 29 &  \model{densenet161} &  93.6 {\footnotesize \textcolor{gray}{[93.3, 93.8]}} &  92.8 {\footnotesize \textcolor{gray}{[92.3, 93.3]}} &  0.8 &  26 &  3 \\
 30 &  \model{resnet101} &  93.5 {\footnotesize \textcolor{gray}{[93.3, 93.8]}} &  92.8 {\footnotesize \textcolor{gray}{[92.3, 93.3]}} &  0.8 &  27 &  3 \\
 31 &  \model{inception\_v3} &  93.5 {\footnotesize \textcolor{gray}{[93.3, 93.7]}} &  92.7 {\footnotesize \textcolor{gray}{[92.1, 93.2]}} &  0.9 &  30 &  1 \\
 32 &  \model{inceptionv3} &  93.4 {\footnotesize \textcolor{gray}{[93.2, 93.6]}} &  92.6 {\footnotesize \textcolor{gray}{[92.1, 93.1]}} &  0.8 &  32 &  0 \\
 33 &  \model{densenet201} &  93.4 {\footnotesize \textcolor{gray}{[93.1, 93.6]}} &  92.4 {\footnotesize \textcolor{gray}{[91.9, 92.9]}} &  1.0 &  33 &  0 \\
 34 &  \model{resnet\_v1\_152\_tf} &  93.2 {\footnotesize \textcolor{gray}{[92.9, 93.4]}} &  92.2 {\footnotesize \textcolor{gray}{[91.7, 92.7]}} &  1.0 &  34 &  0 \\
 35 &  \model{resnet\_v1\_101\_tf} &  92.9 {\footnotesize \textcolor{gray}{[92.7, 93.1]}} &  92.0 {\footnotesize \textcolor{gray}{[91.5, 92.5]}} &  0.9 &  36 &  -1 \\
 36 &  \model{resnet50} &  92.9 {\footnotesize \textcolor{gray}{[92.6, 93.1]}} &  92.0 {\footnotesize \textcolor{gray}{[91.5, 92.5]}} &  0.9 &  37 &  -1 \\
 37 &  \model{resnet\_v2\_50\_tf} &  92.8 {\footnotesize \textcolor{gray}{[92.6, 93.1]}} &  91.9 {\footnotesize \textcolor{gray}{[91.4, 92.5]}} &  0.9 &  38 &  -1 \\
 38 &  \model{densenet169} &  92.8 {\footnotesize \textcolor{gray}{[92.6, 93.0]}} &  91.9 {\footnotesize \textcolor{gray}{[91.4, 92.4]}} &  0.9 &  39 &  -1 \\
 39 &  \model{dpn68} &  92.8 {\footnotesize \textcolor{gray}{[92.5, 93.0]}} &  92.1 {\footnotesize \textcolor{gray}{[91.5, 92.6]}} &  0.7 &  35 &  4 \\
 40 &  \model{cafferesnet101} &  92.8 {\footnotesize \textcolor{gray}{[92.5, 93.0]}} &  91.6 {\footnotesize \textcolor{gray}{[91.1, 92.2]}} &  1.1 &  40 &  0 \\
 41 &  \model{resnet\_v1\_50\_tf} &  92.2 {\footnotesize \textcolor{gray}{[92.0, 92.4]}} &  91.1 {\footnotesize \textcolor{gray}{[90.6, 91.7]}} &  1.0 &  41 &  0 \\
 42 &  \model{densenet121} &  92.0 {\footnotesize \textcolor{gray}{[91.7, 92.2]}} &  91.1 {\footnotesize \textcolor{gray}{[90.5, 91.6]}} &  0.9 &  42 &  0 \\
 43 &  \model{pnasnet\_mobile\_tf} &  91.9 {\footnotesize \textcolor{gray}{[91.6, 92.1]}} &  90.7 {\footnotesize \textcolor{gray}{[90.1, 91.3]}} &  1.1 &  47 &  -4 \\
 44 &  \model{vgg19\_bn} &  91.8 {\footnotesize \textcolor{gray}{[91.6, 92.1]}} &  91.0 {\footnotesize \textcolor{gray}{[90.4, 91.5]}} &  0.9 &  44 &  0 \\
 45 &  \model{inception\_v2\_tf} &  91.8 {\footnotesize \textcolor{gray}{[91.5, 92.0]}} &  91.0 {\footnotesize \textcolor{gray}{[90.5, 91.6]}} &  0.7 &  43 &  2 \\
 46 &  \model{nasnetamobile} &  91.7 {\footnotesize \textcolor{gray}{[91.5, 92.0]}} &  90.9 {\footnotesize \textcolor{gray}{[90.3, 91.4]}} &  0.9 &  46 &  0 \\
 47 &  \model{nasnet\_mobile\_tf} &  91.6 {\footnotesize \textcolor{gray}{[91.3, 91.8]}} &  90.1 {\footnotesize \textcolor{gray}{[89.5, 90.7]}} &  1.4 &  50 &  -3 \\
 48 &  \model{bninception} &  91.6 {\footnotesize \textcolor{gray}{[91.3, 91.8]}} &  90.9 {\footnotesize \textcolor{gray}{[90.3, 91.5]}} &  0.7 &  45 &  3 \\
 49 &  \model{vgg16\_bn} &  91.5 {\footnotesize \textcolor{gray}{[91.3, 91.8]}} &  90.4 {\footnotesize \textcolor{gray}{[89.8, 90.9]}} &  1.1 &  49 &  0 \\
 50 &  \model{resnet34} &  91.4 {\footnotesize \textcolor{gray}{[91.2, 91.7]}} &  90.5 {\footnotesize \textcolor{gray}{[89.9, 91.0]}} &  1.0 &  48 &  2 \\
 51 &  \model{vgg19} &  90.9 {\footnotesize \textcolor{gray}{[90.6, 91.1]}} &  89.7 {\footnotesize \textcolor{gray}{[89.1, 90.3]}} &  1.2 &  51 &  0 \\
 52 &  \model{vgg16} &  90.4 {\footnotesize \textcolor{gray}{[90.1, 90.6]}} &  88.8 {\footnotesize \textcolor{gray}{[88.1, 89.4]}} &  1.6 &  53 &  -1 \\
 53 &  \model{vgg13\_bn} &  90.4 {\footnotesize \textcolor{gray}{[90.1, 90.6]}} &  89.0 {\footnotesize \textcolor{gray}{[88.3, 89.6]}} &  1.4 &  52 &  1 \\
 54 &  \model{mobilenet\_v1\_tf} &  90.0 {\footnotesize \textcolor{gray}{[89.7, 90.2]}} &  87.6 {\footnotesize \textcolor{gray}{[86.9, 88.2]}} &  2.4 &  60 &  -6 \\
 56 &  \model{vgg\_19\_tf} &  89.8 {\footnotesize \textcolor{gray}{[89.6, 90.1]}} &  88.5 {\footnotesize \textcolor{gray}{[87.8, 89.1]}} &  1.4 &  55 &  1 \\
 55 &  \model{vgg\_16\_tf} &  89.8 {\footnotesize \textcolor{gray}{[89.6, 90.1]}} &  88.6 {\footnotesize \textcolor{gray}{[87.9, 89.2]}} &  1.3 &  54 &  1 \\
 57 &  \model{vgg11\_bn} &  89.8 {\footnotesize \textcolor{gray}{[89.5, 90.1]}} &  88.3 {\footnotesize \textcolor{gray}{[87.6, 88.9]}} &  1.5 &  56 &  1 \\
 58 &  \model{inception\_v1\_tf} &  89.6 {\footnotesize \textcolor{gray}{[89.4, 89.9]}} &  88.1 {\footnotesize \textcolor{gray}{[87.4, 88.7]}} &  1.5 &  57 &  1 \\
 59 &  \model{vgg13} &  89.2 {\footnotesize \textcolor{gray}{[89.0, 89.5]}} &  87.6 {\footnotesize \textcolor{gray}{[86.9, 88.2]}} &  1.6 &  59 &  0 \\
 60 &  \model{resnet18} &  89.1 {\footnotesize \textcolor{gray}{[88.8, 89.3]}} &  88.1 {\footnotesize \textcolor{gray}{[87.4, 88.7]}} &  1.0 &  58 &  2 \\
 61 &  \model{vgg11} &  88.6 {\footnotesize \textcolor{gray}{[88.3, 88.9]}} &  86.9 {\footnotesize \textcolor{gray}{[86.2, 87.5]}} &  1.7 &  61 &  0 \\
 62 &  \model{squeezenet1\_1} &  80.6 {\footnotesize \textcolor{gray}{[80.3, 81.0]}} &  78.0 {\footnotesize \textcolor{gray}{[77.2, 78.8]}} &  2.6 &  62 &  0 \\
 63 &  \model{squeezenet1\_0} &  80.4 {\footnotesize \textcolor{gray}{[80.1, 80.8]}} &  77.7 {\footnotesize \textcolor{gray}{[76.9, 78.5]}} &  2.7 &  63 &  0 \\
 64 &  \model{alexnet} &  79.1 {\footnotesize \textcolor{gray}{[78.7, 79.4]}} &  75.9 {\footnotesize \textcolor{gray}{[75.0, 76.7]}} &  3.2 &  64 &  0 \\
 65 &  \model{fv\_64k} &  55.7 {\footnotesize \textcolor{gray}{[55.3, 56.2]}} &  49.8 {\footnotesize \textcolor{gray}{[48.8, 50.7]}} &  6.0 &  65 &  0 \\
 66 &  \model{fv\_16k} &  49.9 {\footnotesize \textcolor{gray}{[49.5, 50.4]}} &  44.2 {\footnotesize \textcolor{gray}{[43.2, 45.2]}} &  5.7 &  66 &  0 \\
 67 &  \model{fv\_4k} &  41.3 {\footnotesize \textcolor{gray}{[40.8, 41.7]}} &  36.5 {\footnotesize \textcolor{gray}{[35.6, 37.5]}} &  4.8 &  67 &  0 \\
\bottomrule
\end{tabular}


==> tables/imagenetv2-b-33_top1_model_results_table.tex <==
\begin{tabular}{rp{4.75cm}rrrrr}
\toprule 
\multicolumn{7}{c}{\textbf{ImageNet Top-1 \datasetb}} \\ 
\midrule
\multicolumn{1}{l}{Orig.} &                               &                                        &                                          &    & \multicolumn{1}{l}{New} &  \\ 
 \multicolumn{1}{l}{Rank} & Model & Orig. Accuracy & New Accuracy & Gap & \multicolumn{1}{l}{Rank} & $\Delta$ Rank \\
\midrule
 1 &  \model{pnasnet\_large\_tf} &  82.9 {\footnotesize \textcolor{gray}{[82.5, 83.2]}} &  72.2 {\footnotesize \textcolor{gray}{[71.3, 73.1]}} &  10.7 &  3 &  -2 \\
 2 &  \model{pnasnet5large} &  82.7 {\footnotesize \textcolor{gray}{[82.4, 83.1]}} &  72.1 {\footnotesize \textcolor{gray}{[71.2, 73.0]}} &  10.7 &  4 &  -2 \\
 3 &  \model{nasnet\_large\_tf} &  82.7 {\footnotesize \textcolor{gray}{[82.4, 83.0]}} &  72.2 {\footnotesize \textcolor{gray}{[71.3, 73.1]}} &  10.5 &  2 &  1 \\
 4 &  \model{nasnetalarge} &  82.5 {\footnotesize \textcolor{gray}{[82.2, 82.8]}} &  72.2 {\footnotesize \textcolor{gray}{[71.3, 73.1]}} &  10.3 &  1 &  3 \\
 5 &  \model{senet154} &  81.3 {\footnotesize \textcolor{gray}{[81.0, 81.6]}} &  70.5 {\footnotesize \textcolor{gray}{[69.6, 71.4]}} &  10.8 &  5 &  0 \\
 6 &  \model{polynet} &  80.9 {\footnotesize \textcolor{gray}{[80.5, 81.2]}} &  70.3 {\footnotesize \textcolor{gray}{[69.4, 71.2]}} &  10.5 &  6 &  0 \\
 7 &  \model{inception\_resnet\_v2\_tf} &  80.4 {\footnotesize \textcolor{gray}{[80.0, 80.7]}} &  69.7 {\footnotesize \textcolor{gray}{[68.7, 70.6]}} &  10.7 &  7 &  0 \\
 8 &  \model{inceptionresnetv2} &  80.3 {\footnotesize \textcolor{gray}{[79.9, 80.6]}} &  69.6 {\footnotesize \textcolor{gray}{[68.7, 70.5]}} &  10.6 &  8 &  0 \\
 9 &  \model{se\_resnext101\_32x4d} &  80.2 {\footnotesize \textcolor{gray}{[79.9, 80.6]}} &  69.3 {\footnotesize \textcolor{gray}{[68.4, 70.2]}} &  10.9 &  9 &  0 \\
 10 &  \model{inception\_v4\_tf} &  80.2 {\footnotesize \textcolor{gray}{[79.8, 80.5]}} &  68.8 {\footnotesize \textcolor{gray}{[67.9, 69.7]}} &  11.4 &  11 &  -1 \\
 11 &  \model{inceptionv4} &  80.1 {\footnotesize \textcolor{gray}{[79.7, 80.4]}} &  69.1 {\footnotesize \textcolor{gray}{[68.2, 70.0]}} &  10.9 &  10 &  1 \\
 12 &  \model{dpn107} &  79.7 {\footnotesize \textcolor{gray}{[79.4, 80.1]}} &  68.1 {\footnotesize \textcolor{gray}{[67.2, 69.0]}} &  11.7 &  12 &  0 \\
 13 &  \model{dpn131} &  79.4 {\footnotesize \textcolor{gray}{[79.1, 79.8]}} &  67.9 {\footnotesize \textcolor{gray}{[67.0, 68.8]}} &  11.5 &  13 &  0 \\
 14 &  \model{dpn92} &  79.4 {\footnotesize \textcolor{gray}{[79.0, 79.8]}} &  67.3 {\footnotesize \textcolor{gray}{[66.3, 68.2]}} &  12.1 &  17 &  -3 \\
 15 &  \model{dpn98} &  79.2 {\footnotesize \textcolor{gray}{[78.9, 79.6]}} &  67.8 {\footnotesize \textcolor{gray}{[66.9, 68.8]}} &  11.4 &  15 &  0 \\
 16 &  \model{se\_resnext50\_32x4d} &  79.1 {\footnotesize \textcolor{gray}{[78.7, 79.4]}} &  67.9 {\footnotesize \textcolor{gray}{[66.9, 68.8]}} &  11.2 &  14 &  2 \\
 17 &  \model{resnext101\_64x4d} &  79.0 {\footnotesize \textcolor{gray}{[78.6, 79.3]}} &  67.1 {\footnotesize \textcolor{gray}{[66.2, 68.0]}} &  11.9 &  20 &  -3 \\
 18 &  \model{xception} &  78.8 {\footnotesize \textcolor{gray}{[78.5, 79.2]}} &  67.2 {\footnotesize \textcolor{gray}{[66.2, 68.1]}} &  11.7 &  18 &  0 \\
 19 &  \model{se\_resnet152} &  78.7 {\footnotesize \textcolor{gray}{[78.3, 79.0]}} &  67.5 {\footnotesize \textcolor{gray}{[66.6, 68.5]}} &  11.1 &  16 &  3 \\
 20 &  \model{se\_resnet101} &  78.4 {\footnotesize \textcolor{gray}{[78.0, 78.8]}} &  67.2 {\footnotesize \textcolor{gray}{[66.2, 68.1]}} &  11.2 &  19 &  1 \\
 21 &  \model{resnet152} &  78.3 {\footnotesize \textcolor{gray}{[77.9, 78.7]}} &  67.0 {\footnotesize \textcolor{gray}{[66.1, 67.9]}} &  11.3 &  21 &  0 \\
 22 &  \model{resnext101\_32x4d} &  78.2 {\footnotesize \textcolor{gray}{[77.8, 78.5]}} &  66.2 {\footnotesize \textcolor{gray}{[65.3, 67.2]}} &  11.9 &  22 &  0 \\
 23 &  \model{inception\_v3\_tf} &  78.0 {\footnotesize \textcolor{gray}{[77.6, 78.3]}} &  66.1 {\footnotesize \textcolor{gray}{[65.1, 67.0]}} &  11.9 &  24 &  -1 \\
 24 &  \model{resnet\_v2\_152\_tf} &  77.8 {\footnotesize \textcolor{gray}{[77.4, 78.1]}} &  66.1 {\footnotesize \textcolor{gray}{[65.1, 67.0]}} &  11.7 &  25 &  -1 \\
 25 &  \model{se\_resnet50} &  77.6 {\footnotesize \textcolor{gray}{[77.3, 78.0]}} &  66.2 {\footnotesize \textcolor{gray}{[65.3, 67.2]}} &  11.4 &  23 &  2 \\
 26 &  \model{fbresnet152} &  77.4 {\footnotesize \textcolor{gray}{[77.0, 77.8]}} &  65.8 {\footnotesize \textcolor{gray}{[64.9, 66.7]}} &  11.6 &  26 &  0 \\
 27 &  \model{resnet101} &  77.4 {\footnotesize \textcolor{gray}{[77.0, 77.7]}} &  65.7 {\footnotesize \textcolor{gray}{[64.7, 66.6]}} &  11.7 &  28 &  -1 \\
 28 &  \model{inceptionv3} &  77.3 {\footnotesize \textcolor{gray}{[77.0, 77.7]}} &  65.7 {\footnotesize \textcolor{gray}{[64.8, 66.7]}} &  11.6 &  27 &  1 \\
 29 &  \model{inception\_v3} &  77.2 {\footnotesize \textcolor{gray}{[76.8, 77.6]}} &  65.4 {\footnotesize \textcolor{gray}{[64.5, 66.4]}} &  11.8 &  29 &  0 \\
 30 &  \model{densenet161} &  77.1 {\footnotesize \textcolor{gray}{[76.8, 77.5]}} &  65.3 {\footnotesize \textcolor{gray}{[64.4, 66.2]}} &  11.8 &  30 &  0 \\
 31 &  \model{dpn68b} &  77.0 {\footnotesize \textcolor{gray}{[76.7, 77.4]}} &  64.7 {\footnotesize \textcolor{gray}{[63.7, 65.6]}} &  12.4 &  32 &  -1 \\
 32 &  \model{resnet\_v2\_101\_tf} &  77.0 {\footnotesize \textcolor{gray}{[76.6, 77.3]}} &  64.6 {\footnotesize \textcolor{gray}{[63.7, 65.6]}} &  12.3 &  34 &  -2 \\
 33 &  \model{densenet201} &  76.9 {\footnotesize \textcolor{gray}{[76.5, 77.3]}} &  64.7 {\footnotesize \textcolor{gray}{[63.7, 65.6]}} &  12.2 &  31 &  2 \\
 34 &  \model{resnet\_v1\_152\_tf} &  76.8 {\footnotesize \textcolor{gray}{[76.4, 77.2]}} &  64.6 {\footnotesize \textcolor{gray}{[63.7, 65.6]}} &  12.2 &  33 &  1 \\
 35 &  \model{resnet\_v1\_101\_tf} &  76.4 {\footnotesize \textcolor{gray}{[76.0, 76.8]}} &  64.5 {\footnotesize \textcolor{gray}{[63.6, 65.5]}} &  11.9 &  35 &  0 \\
 36 &  \model{cafferesnet101} &  76.2 {\footnotesize \textcolor{gray}{[75.8, 76.6]}} &  64.3 {\footnotesize \textcolor{gray}{[63.4, 65.2]}} &  11.9 &  36 &  0 \\
 37 &  \model{resnet50} &  76.1 {\footnotesize \textcolor{gray}{[75.8, 76.5]}} &  63.3 {\footnotesize \textcolor{gray}{[62.4, 64.3]}} &  12.8 &  39 &  -2 \\
 38 &  \model{dpn68} &  75.9 {\footnotesize \textcolor{gray}{[75.5, 76.2]}} &  63.4 {\footnotesize \textcolor{gray}{[62.5, 64.4]}} &  12.4 &  38 &  0 \\
 39 &  \model{densenet169} &  75.6 {\footnotesize \textcolor{gray}{[75.2, 76.0]}} &  63.9 {\footnotesize \textcolor{gray}{[62.9, 64.8]}} &  11.7 &  37 &  2 \\
 40 &  \model{resnet\_v2\_50\_tf} &  75.6 {\footnotesize \textcolor{gray}{[75.2, 76.0]}} &  62.7 {\footnotesize \textcolor{gray}{[61.8, 63.7]}} &  12.9 &  40 &  0 \\
 41 &  \model{resnet\_v1\_50\_tf} &  75.2 {\footnotesize \textcolor{gray}{[74.8, 75.6]}} &  62.6 {\footnotesize \textcolor{gray}{[61.6, 63.5]}} &  12.6 &  41 &  0 \\
 42 &  \model{densenet121} &  74.4 {\footnotesize \textcolor{gray}{[74.0, 74.8]}} &  62.2 {\footnotesize \textcolor{gray}{[61.3, 63.2]}} &  12.2 &  42 &  0 \\
 43 &  \model{vgg19\_bn} &  74.2 {\footnotesize \textcolor{gray}{[73.8, 74.6]}} &  61.9 {\footnotesize \textcolor{gray}{[60.9, 62.8]}} &  12.3 &  44 &  -1 \\
 44 &  \model{pnasnet\_mobile\_tf} &  74.1 {\footnotesize \textcolor{gray}{[73.8, 74.5]}} &  60.9 {\footnotesize \textcolor{gray}{[59.9, 61.8]}} &  13.3 &  48 &  -4 \\
 45 &  \model{nasnetamobile} &  74.1 {\footnotesize \textcolor{gray}{[73.7, 74.5]}} &  61.6 {\footnotesize \textcolor{gray}{[60.6, 62.5]}} &  12.5 &  45 &  0 \\
 46 &  \model{inception\_v2\_tf} &  74.0 {\footnotesize \textcolor{gray}{[73.6, 74.4]}} &  61.2 {\footnotesize \textcolor{gray}{[60.2, 62.2]}} &  12.8 &  46 &  0 \\
 47 &  \model{nasnet\_mobile\_tf} &  74.0 {\footnotesize \textcolor{gray}{[73.6, 74.4]}} &  60.8 {\footnotesize \textcolor{gray}{[59.8, 61.7]}} &  13.2 &  50 &  -3 \\
 48 &  \model{bninception} &  73.5 {\footnotesize \textcolor{gray}{[73.1, 73.9]}} &  62.1 {\footnotesize \textcolor{gray}{[61.2, 63.1]}} &  11.4 &  43 &  5 \\
 49 &  \model{vgg16\_bn} &  73.4 {\footnotesize \textcolor{gray}{[73.0, 73.7]}} &  60.8 {\footnotesize \textcolor{gray}{[59.8, 61.7]}} &  12.6 &  49 &  0 \\
 50 &  \model{resnet34} &  73.3 {\footnotesize \textcolor{gray}{[72.9, 73.7]}} &  61.2 {\footnotesize \textcolor{gray}{[60.2, 62.2]}} &  12.1 &  47 &  3 \\
 51 &  \model{vgg19} &  72.4 {\footnotesize \textcolor{gray}{[72.0, 72.8]}} &  59.7 {\footnotesize \textcolor{gray}{[58.7, 60.7]}} &  12.7 &  51 &  0 \\
 52 &  \model{vgg16} &  71.6 {\footnotesize \textcolor{gray}{[71.2, 72.0]}} &  58.8 {\footnotesize \textcolor{gray}{[57.9, 59.8]}} &  12.8 &  53 &  -1 \\
 53 &  \model{vgg13\_bn} &  71.6 {\footnotesize \textcolor{gray}{[71.2, 72.0]}} &  59.0 {\footnotesize \textcolor{gray}{[58.0, 59.9]}} &  12.6 &  52 &  1 \\
 54 &  \model{mobilenet\_v1\_tf} &  71.0 {\footnotesize \textcolor{gray}{[70.6, 71.4]}} &  57.4 {\footnotesize \textcolor{gray}{[56.4, 58.4]}} &  13.6 &  56 &  -2 \\
 55 &  \model{vgg\_19\_tf} &  71.0 {\footnotesize \textcolor{gray}{[70.6, 71.4]}} &  58.6 {\footnotesize \textcolor{gray}{[57.7, 59.6]}} &  12.4 &  54 &  1 \\
 56 &  \model{vgg\_16\_tf} &  70.9 {\footnotesize \textcolor{gray}{[70.5, 71.3]}} &  58.4 {\footnotesize \textcolor{gray}{[57.4, 59.3]}} &  12.5 &  55 &  1 \\
 57 &  \model{vgg11\_bn} &  70.4 {\footnotesize \textcolor{gray}{[70.0, 70.8]}} &  57.4 {\footnotesize \textcolor{gray}{[56.4, 58.4]}} &  13.0 &  57 &  0 \\
 58 &  \model{vgg13} &  69.9 {\footnotesize \textcolor{gray}{[69.5, 70.3]}} &  57.1 {\footnotesize \textcolor{gray}{[56.2, 58.1]}} &  12.8 &  59 &  -1 \\
 59 &  \model{inception\_v1\_tf} &  69.8 {\footnotesize \textcolor{gray}{[69.4, 70.2]}} &  56.6 {\footnotesize \textcolor{gray}{[55.7, 57.6]}} &  13.1 &  60 &  -1 \\
 60 &  \model{resnet18} &  69.8 {\footnotesize \textcolor{gray}{[69.4, 70.2]}} &  57.2 {\footnotesize \textcolor{gray}{[56.2, 58.2]}} &  12.6 &  58 &  2 \\
 61 &  \model{vgg11} &  69.0 {\footnotesize \textcolor{gray}{[68.6, 69.4]}} &  55.8 {\footnotesize \textcolor{gray}{[54.8, 56.8]}} &  13.2 &  61 &  0 \\
 62 &  \model{squeezenet1\_1} &  58.2 {\footnotesize \textcolor{gray}{[57.7, 58.6]}} &  45.3 {\footnotesize \textcolor{gray}{[44.4, 46.3]}} &  12.8 &  62 &  0 \\
 63 &  \model{squeezenet1\_0} &  58.1 {\footnotesize \textcolor{gray}{[57.7, 58.5]}} &  45.0 {\footnotesize \textcolor{gray}{[44.0, 46.0]}} &  13.1 &  63 &  0 \\
 64 &  \model{alexnet} &  56.5 {\footnotesize \textcolor{gray}{[56.1, 57.0]}} &  44.0 {\footnotesize \textcolor{gray}{[43.0, 45.0]}} &  12.5 &  64 &  0 \\
 65 &  \model{fv\_64k} &  35.1 {\footnotesize \textcolor{gray}{[34.7, 35.5]}} &  24.1 {\footnotesize \textcolor{gray}{[23.2, 24.9]}} &  11.0 &  65 &  0 \\
 66 &  \model{fv\_16k} &  28.3 {\footnotesize \textcolor{gray}{[27.9, 28.7]}} &  19.2 {\footnotesize \textcolor{gray}{[18.5, 20.0]}} &  9.1 &  66 &  0 \\
 67 &  \model{fv\_4k} &  21.2 {\footnotesize \textcolor{gray}{[20.8, 21.5]}} &  15.0 {\footnotesize \textcolor{gray}{[14.3, 15.7]}} &  6.2 &  67 &  0 \\
\bottomrule
\end{tabular}


==> tables/imagenetv2-b-33_top5_model_results_table.tex <==
\begin{tabular}{rp{4.75cm}rrrrr}
\toprule 
\multicolumn{7}{c}{\textbf{ImageNet Top-5 \datasetb}} \\ 
\midrule
\multicolumn{1}{l}{Orig.} &                               &                                        &                                          &    & \multicolumn{1}{l}{New} &  \\ 
 \multicolumn{1}{l}{Rank} & Model & Orig. Accuracy & New Accuracy & Gap & \multicolumn{1}{l}{Rank} & $\Delta$ Rank \\
\midrule
 1 &  \model{pnasnet\_large\_tf} &  96.2 {\footnotesize \textcolor{gray}{[96.0, 96.3]}} &  90.1 {\footnotesize \textcolor{gray}{[89.5, 90.7]}} &  6.1 &  3 &  -2 \\
 2 &  \model{nasnet\_large\_tf} &  96.2 {\footnotesize \textcolor{gray}{[96.0, 96.3]}} &  90.1 {\footnotesize \textcolor{gray}{[89.5, 90.6]}} &  6.1 &  4 &  -2 \\
 3 &  \model{nasnetalarge} &  96.0 {\footnotesize \textcolor{gray}{[95.8, 96.2]}} &  90.4 {\footnotesize \textcolor{gray}{[89.8, 91.0]}} &  5.6 &  1 &  2 \\
 4 &  \model{pnasnet5large} &  96.0 {\footnotesize \textcolor{gray}{[95.8, 96.2]}} &  90.2 {\footnotesize \textcolor{gray}{[89.6, 90.8]}} &  5.8 &  2 &  2 \\
 5 &  \model{polynet} &  95.6 {\footnotesize \textcolor{gray}{[95.4, 95.7]}} &  89.1 {\footnotesize \textcolor{gray}{[88.5, 89.7]}} &  6.4 &  5 &  0 \\
 6 &  \model{senet154} &  95.5 {\footnotesize \textcolor{gray}{[95.3, 95.7]}} &  89.0 {\footnotesize \textcolor{gray}{[88.4, 89.6]}} &  6.5 &  6 &  0 \\
 7 &  \model{inception\_resnet\_v2\_tf} &  95.2 {\footnotesize \textcolor{gray}{[95.1, 95.4]}} &  88.4 {\footnotesize \textcolor{gray}{[87.7, 89.0]}} &  6.9 &  9 &  -2 \\
 8 &  \model{inception\_v4\_tf} &  95.2 {\footnotesize \textcolor{gray}{[95.0, 95.4]}} &  88.3 {\footnotesize \textcolor{gray}{[87.6, 88.9]}} &  6.9 &  10 &  -2 \\
 9 &  \model{inceptionresnetv2} &  95.1 {\footnotesize \textcolor{gray}{[94.9, 95.3]}} &  88.5 {\footnotesize \textcolor{gray}{[87.8, 89.1]}} &  6.7 &  8 &  1 \\
 10 &  \model{se\_resnext101\_32x4d} &  95.0 {\footnotesize \textcolor{gray}{[94.8, 95.2]}} &  88.0 {\footnotesize \textcolor{gray}{[87.4, 88.7]}} &  7.0 &  11 &  -1 \\
 11 &  \model{inceptionv4} &  94.9 {\footnotesize \textcolor{gray}{[94.7, 95.1]}} &  88.7 {\footnotesize \textcolor{gray}{[88.1, 89.3]}} &  6.2 &  7 &  4 \\
 12 &  \model{dpn107} &  94.7 {\footnotesize \textcolor{gray}{[94.5, 94.9]}} &  87.6 {\footnotesize \textcolor{gray}{[86.9, 88.2]}} &  7.1 &  13 &  -1 \\
 13 &  \model{dpn92} &  94.6 {\footnotesize \textcolor{gray}{[94.4, 94.8]}} &  87.2 {\footnotesize \textcolor{gray}{[86.5, 87.8]}} &  7.5 &  17 &  -4 \\
 14 &  \model{dpn131} &  94.6 {\footnotesize \textcolor{gray}{[94.4, 94.8]}} &  87.0 {\footnotesize \textcolor{gray}{[86.3, 87.7]}} &  7.6 &  19 &  -5 \\
 15 &  \model{dpn98} &  94.5 {\footnotesize \textcolor{gray}{[94.3, 94.7]}} &  87.2 {\footnotesize \textcolor{gray}{[86.5, 87.8]}} &  7.3 &  16 &  -1 \\
 16 &  \model{se\_resnext50\_32x4d} &  94.4 {\footnotesize \textcolor{gray}{[94.2, 94.6]}} &  87.6 {\footnotesize \textcolor{gray}{[87.0, 88.3]}} &  6.8 &  12 &  4 \\
 17 &  \model{se\_resnet152} &  94.4 {\footnotesize \textcolor{gray}{[94.2, 94.6]}} &  87.4 {\footnotesize \textcolor{gray}{[86.7, 88.0]}} &  7.0 &  15 &  2 \\
 18 &  \model{xception} &  94.3 {\footnotesize \textcolor{gray}{[94.1, 94.5]}} &  87.0 {\footnotesize \textcolor{gray}{[86.3, 87.7]}} &  7.3 &  20 &  -2 \\
 19 &  \model{se\_resnet101} &  94.3 {\footnotesize \textcolor{gray}{[94.1, 94.5]}} &  87.1 {\footnotesize \textcolor{gray}{[86.4, 87.7]}} &  7.2 &  18 &  1 \\
 20 &  \model{resnext101\_64x4d} &  94.3 {\footnotesize \textcolor{gray}{[94.0, 94.5]}} &  86.9 {\footnotesize \textcolor{gray}{[86.2, 87.5]}} &  7.4 &  22 &  -2 \\
 21 &  \model{resnet\_v2\_152\_tf} &  94.1 {\footnotesize \textcolor{gray}{[93.9, 94.3]}} &  86.9 {\footnotesize \textcolor{gray}{[86.2, 87.5]}} &  7.2 &  21 &  0 \\
 22 &  \model{resnet152} &  94.0 {\footnotesize \textcolor{gray}{[93.8, 94.3]}} &  87.6 {\footnotesize \textcolor{gray}{[86.9, 88.2]}} &  6.5 &  14 &  8 \\
 23 &  \model{inception\_v3\_tf} &  93.9 {\footnotesize \textcolor{gray}{[93.7, 94.1]}} &  86.4 {\footnotesize \textcolor{gray}{[85.7, 87.0]}} &  7.6 &  23 &  0 \\
 24 &  \model{resnext101\_32x4d} &  93.9 {\footnotesize \textcolor{gray}{[93.7, 94.1]}} &  86.2 {\footnotesize \textcolor{gray}{[85.5, 86.8]}} &  7.7 &  25 &  -1 \\
 25 &  \model{se\_resnet50} &  93.8 {\footnotesize \textcolor{gray}{[93.5, 94.0]}} &  86.3 {\footnotesize \textcolor{gray}{[85.6, 87.0]}} &  7.4 &  24 &  1 \\
 26 &  \model{resnet\_v2\_101\_tf} &  93.7 {\footnotesize \textcolor{gray}{[93.5, 93.9]}} &  86.1 {\footnotesize \textcolor{gray}{[85.4, 86.8]}} &  7.6 &  27 &  -1 \\
 27 &  \model{fbresnet152} &  93.6 {\footnotesize \textcolor{gray}{[93.4, 93.8]}} &  86.1 {\footnotesize \textcolor{gray}{[85.4, 86.7]}} &  7.5 &  28 &  -1 \\
 28 &  \model{dpn68b} &  93.6 {\footnotesize \textcolor{gray}{[93.4, 93.8]}} &  85.3 {\footnotesize \textcolor{gray}{[84.6, 86.0]}} &  8.3 &  33 &  -5 \\
 29 &  \model{densenet161} &  93.6 {\footnotesize \textcolor{gray}{[93.3, 93.8]}} &  86.1 {\footnotesize \textcolor{gray}{[85.4, 86.8]}} &  7.4 &  26 &  3 \\
 30 &  \model{resnet101} &  93.5 {\footnotesize \textcolor{gray}{[93.3, 93.8]}} &  86.0 {\footnotesize \textcolor{gray}{[85.3, 86.7]}} &  7.6 &  30 &  0 \\
 31 &  \model{inception\_v3} &  93.5 {\footnotesize \textcolor{gray}{[93.3, 93.7]}} &  85.9 {\footnotesize \textcolor{gray}{[85.2, 86.6]}} &  7.6 &  31 &  0 \\
 32 &  \model{inceptionv3} &  93.4 {\footnotesize \textcolor{gray}{[93.2, 93.6]}} &  86.1 {\footnotesize \textcolor{gray}{[85.4, 86.7]}} &  7.4 &  29 &  3 \\
 33 &  \model{densenet201} &  93.4 {\footnotesize \textcolor{gray}{[93.1, 93.6]}} &  85.3 {\footnotesize \textcolor{gray}{[84.6, 86.0]}} &  8.1 &  34 &  -1 \\
 34 &  \model{resnet\_v1\_152\_tf} &  93.2 {\footnotesize \textcolor{gray}{[92.9, 93.4]}} &  85.4 {\footnotesize \textcolor{gray}{[84.6, 86.0]}} &  7.8 &  32 &  2 \\
 35 &  \model{resnet\_v1\_101\_tf} &  92.9 {\footnotesize \textcolor{gray}{[92.7, 93.1]}} &  85.2 {\footnotesize \textcolor{gray}{[84.5, 85.9]}} &  7.7 &  35 &  0 \\
 36 &  \model{resnet50} &  92.9 {\footnotesize \textcolor{gray}{[92.6, 93.1]}} &  84.7 {\footnotesize \textcolor{gray}{[83.9, 85.4]}} &  8.2 &  38 &  -2 \\
 37 &  \model{resnet\_v2\_50\_tf} &  92.8 {\footnotesize \textcolor{gray}{[92.6, 93.1]}} &  84.4 {\footnotesize \textcolor{gray}{[83.6, 85.1]}} &  8.5 &  40 &  -3 \\
 38 &  \model{densenet169} &  92.8 {\footnotesize \textcolor{gray}{[92.6, 93.0]}} &  84.7 {\footnotesize \textcolor{gray}{[84.0, 85.4]}} &  8.1 &  37 &  1 \\
 39 &  \model{dpn68} &  92.8 {\footnotesize \textcolor{gray}{[92.5, 93.0]}} &  84.6 {\footnotesize \textcolor{gray}{[83.9, 85.3]}} &  8.2 &  39 &  0 \\
 40 &  \model{cafferesnet101} &  92.8 {\footnotesize \textcolor{gray}{[92.5, 93.0]}} &  84.9 {\footnotesize \textcolor{gray}{[84.1, 85.6]}} &  7.9 &  36 &  4 \\
 41 &  \model{resnet\_v1\_50\_tf} &  92.2 {\footnotesize \textcolor{gray}{[92.0, 92.4]}} &  84.1 {\footnotesize \textcolor{gray}{[83.4, 84.8]}} &  8.1 &  41 &  0 \\
 42 &  \model{densenet121} &  92.0 {\footnotesize \textcolor{gray}{[91.7, 92.2]}} &  83.8 {\footnotesize \textcolor{gray}{[83.1, 84.5]}} &  8.2 &  42 &  0 \\
 43 &  \model{pnasnet\_mobile\_tf} &  91.9 {\footnotesize \textcolor{gray}{[91.6, 92.1]}} &  83.1 {\footnotesize \textcolor{gray}{[82.4, 83.8]}} &  8.8 &  46 &  -3 \\
 44 &  \model{vgg19\_bn} &  91.8 {\footnotesize \textcolor{gray}{[91.6, 92.1]}} &  83.5 {\footnotesize \textcolor{gray}{[82.7, 84.2]}} &  8.4 &  43 &  1 \\
 45 &  \model{inception\_v2\_tf} &  91.8 {\footnotesize \textcolor{gray}{[91.5, 92.0]}} &  83.1 {\footnotesize \textcolor{gray}{[82.3, 83.8]}} &  8.7 &  47 &  -2 \\
 46 &  \model{nasnetamobile} &  91.7 {\footnotesize \textcolor{gray}{[91.5, 92.0]}} &  83.4 {\footnotesize \textcolor{gray}{[82.6, 84.1]}} &  8.4 &  45 &  1 \\
 47 &  \model{nasnet\_mobile\_tf} &  91.6 {\footnotesize \textcolor{gray}{[91.3, 91.8]}} &  82.2 {\footnotesize \textcolor{gray}{[81.4, 82.9]}} &  9.4 &  50 &  -3 \\
 48 &  \model{bninception} &  91.6 {\footnotesize \textcolor{gray}{[91.3, 91.8]}} &  83.4 {\footnotesize \textcolor{gray}{[82.7, 84.2]}} &  8.1 &  44 &  4 \\
 49 &  \model{vgg16\_bn} &  91.5 {\footnotesize \textcolor{gray}{[91.3, 91.8]}} &  83.0 {\footnotesize \textcolor{gray}{[82.2, 83.7]}} &  8.6 &  48 &  1 \\
 50 &  \model{resnet34} &  91.4 {\footnotesize \textcolor{gray}{[91.2, 91.7]}} &  82.7 {\footnotesize \textcolor{gray}{[82.0, 83.5]}} &  8.7 &  49 &  1 \\
 51 &  \model{vgg19} &  90.9 {\footnotesize \textcolor{gray}{[90.6, 91.1]}} &  81.5 {\footnotesize \textcolor{gray}{[80.7, 82.2]}} &  9.4 &  52 &  -1 \\
 52 &  \model{vgg16} &  90.4 {\footnotesize \textcolor{gray}{[90.1, 90.6]}} &  81.7 {\footnotesize \textcolor{gray}{[80.9, 82.4]}} &  8.7 &  51 &  1 \\
 53 &  \model{vgg13\_bn} &  90.4 {\footnotesize \textcolor{gray}{[90.1, 90.6]}} &  81.1 {\footnotesize \textcolor{gray}{[80.3, 81.9]}} &  9.3 &  53 &  0 \\
 54 &  \model{mobilenet\_v1\_tf} &  90.0 {\footnotesize \textcolor{gray}{[89.7, 90.2]}} &  79.4 {\footnotesize \textcolor{gray}{[78.6, 80.1]}} &  10.6 &  60 &  -6 \\
 56 &  \model{vgg\_19\_tf} &  89.8 {\footnotesize \textcolor{gray}{[89.6, 90.1]}} &  80.7 {\footnotesize \textcolor{gray}{[79.9, 81.4]}} &  9.2 &  54 &  2 \\
 55 &  \model{vgg\_16\_tf} &  89.8 {\footnotesize \textcolor{gray}{[89.6, 90.1]}} &  80.5 {\footnotesize \textcolor{gray}{[79.7, 81.3]}} &  9.3 &  55 &  0 \\
 57 &  \model{vgg11\_bn} &  89.8 {\footnotesize \textcolor{gray}{[89.5, 90.1]}} &  80.0 {\footnotesize \textcolor{gray}{[79.2, 80.8]}} &  9.8 &  58 &  -1 \\
 58 &  \model{inception\_v1\_tf} &  89.6 {\footnotesize \textcolor{gray}{[89.4, 89.9]}} &  80.1 {\footnotesize \textcolor{gray}{[79.3, 80.9]}} &  9.5 &  57 &  1 \\
 59 &  \model{vgg13} &  89.2 {\footnotesize \textcolor{gray}{[89.0, 89.5]}} &  79.5 {\footnotesize \textcolor{gray}{[78.7, 80.3]}} &  9.7 &  59 &  0 \\
 60 &  \model{resnet18} &  89.1 {\footnotesize \textcolor{gray}{[88.8, 89.3]}} &  80.2 {\footnotesize \textcolor{gray}{[79.4, 81.0]}} &  8.9 &  56 &  4 \\
 61 &  \model{vgg11} &  88.6 {\footnotesize \textcolor{gray}{[88.3, 88.9]}} &  78.8 {\footnotesize \textcolor{gray}{[78.0, 79.6]}} &  9.8 &  61 &  0 \\
 62 &  \model{squeezenet1\_1} &  80.6 {\footnotesize \textcolor{gray}{[80.3, 81.0]}} &  69.0 {\footnotesize \textcolor{gray}{[68.1, 69.9]}} &  11.6 &  62 &  0 \\
 63 &  \model{squeezenet1\_0} &  80.4 {\footnotesize \textcolor{gray}{[80.1, 80.8]}} &  68.5 {\footnotesize \textcolor{gray}{[67.6, 69.4]}} &  11.9 &  63 &  0 \\
 64 &  \model{alexnet} &  79.1 {\footnotesize \textcolor{gray}{[78.7, 79.4]}} &  67.4 {\footnotesize \textcolor{gray}{[66.5, 68.3]}} &  11.7 &  64 &  0 \\
 65 &  \model{fv\_64k} &  55.7 {\footnotesize \textcolor{gray}{[55.3, 56.2]}} &  42.6 {\footnotesize \textcolor{gray}{[41.6, 43.6]}} &  13.2 &  65 &  0 \\
 66 &  \model{fv\_16k} &  49.9 {\footnotesize \textcolor{gray}{[49.5, 50.4]}} &  37.5 {\footnotesize \textcolor{gray}{[36.6, 38.5]}} &  12.4 &  66 &  0 \\
 67 &  \model{fv\_4k} &  41.3 {\footnotesize \textcolor{gray}{[40.8, 41.7]}} &  31.0 {\footnotesize \textcolor{gray}{[30.1, 31.9]}} &  10.3 &  67 &  0 \\
\bottomrule
\end{tabular}


==> tables/imagenetv2-c-12_top1_model_results_table.tex <==
\begin{tabular}{rp{4.75cm}rrrrr}
\toprule 
\multicolumn{7}{c}{\textbf{ImageNet Top-1 \datasetc}} \\ 
\midrule
\multicolumn{1}{l}{Orig.} &                               &                                        &                                          &    & \multicolumn{1}{l}{New} &  \\ 
 \multicolumn{1}{l}{Rank} & Model & Orig. Accuracy & New Accuracy & Gap & \multicolumn{1}{l}{Rank} & $\Delta$ Rank \\
\midrule
 1 &  \model{pnasnet\_large\_tf} &  82.9 {\footnotesize \textcolor{gray}{[82.5, 83.2]}} &  83.9 {\footnotesize \textcolor{gray}{[83.2, 84.6]}} &  -1.0 &  3 &  -2 \\
 2 &  \model{pnasnet5large} &  82.7 {\footnotesize \textcolor{gray}{[82.4, 83.1]}} &  83.9 {\footnotesize \textcolor{gray}{[83.1, 84.6]}} &  -1.1 &  4 &  -2 \\
 3 &  \model{nasnet\_large\_tf} &  82.7 {\footnotesize \textcolor{gray}{[82.4, 83.0]}} &  84.0 {\footnotesize \textcolor{gray}{[83.3, 84.7]}} &  -1.3 &  2 &  1 \\
 4 &  \model{nasnetalarge} &  82.5 {\footnotesize \textcolor{gray}{[82.2, 82.8]}} &  84.2 {\footnotesize \textcolor{gray}{[83.4, 84.9]}} &  -1.7 &  1 &  3 \\
 5 &  \model{senet154} &  81.3 {\footnotesize \textcolor{gray}{[81.0, 81.6]}} &  82.8 {\footnotesize \textcolor{gray}{[82.1, 83.6]}} &  -1.5 &  6 &  -1 \\
 6 &  \model{polynet} &  80.9 {\footnotesize \textcolor{gray}{[80.5, 81.2]}} &  83.0 {\footnotesize \textcolor{gray}{[82.2, 83.7]}} &  -2.1 &  5 &  1 \\
 7 &  \model{inception\_resnet\_v2\_tf} &  80.4 {\footnotesize \textcolor{gray}{[80.0, 80.7]}} &  82.5 {\footnotesize \textcolor{gray}{[81.7, 83.2]}} &  -2.1 &  8 &  -1 \\
 8 &  \model{inceptionresnetv2} &  80.3 {\footnotesize \textcolor{gray}{[79.9, 80.6]}} &  82.8 {\footnotesize \textcolor{gray}{[82.0, 83.5]}} &  -2.5 &  7 &  1 \\
 9 &  \model{se\_resnext101\_32x4d} &  80.2 {\footnotesize \textcolor{gray}{[79.9, 80.6]}} &  82.2 {\footnotesize \textcolor{gray}{[81.5, 83.0]}} &  -2.0 &  11 &  -2 \\
 10 &  \model{inception\_v4\_tf} &  80.2 {\footnotesize \textcolor{gray}{[79.8, 80.5]}} &  82.3 {\footnotesize \textcolor{gray}{[81.5, 83.0]}} &  -2.1 &  9 &  1 \\
 11 &  \model{inceptionv4} &  80.1 {\footnotesize \textcolor{gray}{[79.7, 80.4]}} &  82.3 {\footnotesize \textcolor{gray}{[81.5, 83.0]}} &  -2.2 &  10 &  1 \\
 12 &  \model{dpn107} &  79.7 {\footnotesize \textcolor{gray}{[79.4, 80.1]}} &  81.4 {\footnotesize \textcolor{gray}{[80.6, 82.1]}} &  -1.6 &  13 &  -1 \\
 13 &  \model{dpn131} &  79.4 {\footnotesize \textcolor{gray}{[79.1, 79.8]}} &  81.3 {\footnotesize \textcolor{gray}{[80.5, 82.1]}} &  -1.9 &  15 &  -2 \\
 14 &  \model{dpn92} &  79.4 {\footnotesize \textcolor{gray}{[79.0, 79.8]}} &  81.2 {\footnotesize \textcolor{gray}{[80.5, 82.0]}} &  -1.8 &  16 &  -2 \\
 15 &  \model{dpn98} &  79.2 {\footnotesize \textcolor{gray}{[78.9, 79.6]}} &  81.5 {\footnotesize \textcolor{gray}{[80.7, 82.3]}} &  -2.3 &  12 &  3 \\
 16 &  \model{se\_resnext50\_32x4d} &  79.1 {\footnotesize \textcolor{gray}{[78.7, 79.4]}} &  81.4 {\footnotesize \textcolor{gray}{[80.6, 82.1]}} &  -2.3 &  14 &  2 \\
 17 &  \model{resnext101\_64x4d} &  79.0 {\footnotesize \textcolor{gray}{[78.6, 79.3]}} &  80.3 {\footnotesize \textcolor{gray}{[79.5, 81.0]}} &  -1.3 &  22 &  -5 \\
 18 &  \model{xception} &  78.8 {\footnotesize \textcolor{gray}{[78.5, 79.2]}} &  81.0 {\footnotesize \textcolor{gray}{[80.2, 81.8]}} &  -2.2 &  18 &  0 \\
 19 &  \model{se\_resnet152} &  78.7 {\footnotesize \textcolor{gray}{[78.3, 79.0]}} &  81.0 {\footnotesize \textcolor{gray}{[80.3, 81.8]}} &  -2.4 &  17 &  2 \\
 20 &  \model{se\_resnet101} &  78.4 {\footnotesize \textcolor{gray}{[78.0, 78.8]}} &  80.5 {\footnotesize \textcolor{gray}{[79.7, 81.3]}} &  -2.1 &  19 &  1 \\
 21 &  \model{resnet152} &  78.3 {\footnotesize \textcolor{gray}{[77.9, 78.7]}} &  80.3 {\footnotesize \textcolor{gray}{[79.5, 81.1]}} &  -2.0 &  21 &  0 \\
 22 &  \model{resnext101\_32x4d} &  78.2 {\footnotesize \textcolor{gray}{[77.8, 78.5]}} &  79.9 {\footnotesize \textcolor{gray}{[79.1, 80.6]}} &  -1.7 &  26 &  -4 \\
 23 &  \model{inception\_v3\_tf} &  78.0 {\footnotesize \textcolor{gray}{[77.6, 78.3]}} &  80.1 {\footnotesize \textcolor{gray}{[79.3, 80.9]}} &  -2.1 &  23 &  0 \\
 24 &  \model{resnet\_v2\_152\_tf} &  77.8 {\footnotesize \textcolor{gray}{[77.4, 78.1]}} &  80.3 {\footnotesize \textcolor{gray}{[79.5, 81.1]}} &  -2.6 &  20 &  4 \\
 25 &  \model{se\_resnet50} &  77.6 {\footnotesize \textcolor{gray}{[77.3, 78.0]}} &  79.4 {\footnotesize \textcolor{gray}{[78.6, 80.2]}} &  -1.8 &  31 &  -6 \\
 26 &  \model{fbresnet152} &  77.4 {\footnotesize \textcolor{gray}{[77.0, 77.8]}} &  80.1 {\footnotesize \textcolor{gray}{[79.3, 80.9]}} &  -2.7 &  24 &  2 \\
 27 &  \model{resnet101} &  77.4 {\footnotesize \textcolor{gray}{[77.0, 77.7]}} &  79.0 {\footnotesize \textcolor{gray}{[78.2, 79.8]}} &  -1.7 &  32 &  -5 \\
 28 &  \model{inceptionv3} &  77.3 {\footnotesize \textcolor{gray}{[77.0, 77.7]}} &  79.6 {\footnotesize \textcolor{gray}{[78.8, 80.4]}} &  -2.3 &  27 &  1 \\
 29 &  \model{inception\_v3} &  77.2 {\footnotesize \textcolor{gray}{[76.8, 77.6]}} &  79.6 {\footnotesize \textcolor{gray}{[78.8, 80.4]}} &  -2.4 &  28 &  1 \\
 30 &  \model{densenet161} &  77.1 {\footnotesize \textcolor{gray}{[76.8, 77.5]}} &  79.5 {\footnotesize \textcolor{gray}{[78.7, 80.3]}} &  -2.4 &  29 &  1 \\
 31 &  \model{dpn68b} &  77.0 {\footnotesize \textcolor{gray}{[76.7, 77.4]}} &  79.4 {\footnotesize \textcolor{gray}{[78.6, 80.2]}} &  -2.4 &  30 &  1 \\
 32 &  \model{resnet\_v2\_101\_tf} &  77.0 {\footnotesize \textcolor{gray}{[76.6, 77.3]}} &  80.1 {\footnotesize \textcolor{gray}{[79.3, 80.8]}} &  -3.1 &  25 &  7 \\
 33 &  \model{densenet201} &  76.9 {\footnotesize \textcolor{gray}{[76.5, 77.3]}} &  79.0 {\footnotesize \textcolor{gray}{[78.1, 79.7]}} &  -2.1 &  34 &  -1 \\
 34 &  \model{resnet\_v1\_152\_tf} &  76.8 {\footnotesize \textcolor{gray}{[76.4, 77.2]}} &  79.0 {\footnotesize \textcolor{gray}{[78.2, 79.8]}} &  -2.2 &  33 &  1 \\
 35 &  \model{resnet\_v1\_101\_tf} &  76.4 {\footnotesize \textcolor{gray}{[76.0, 76.8]}} &  78.6 {\footnotesize \textcolor{gray}{[77.8, 79.4]}} &  -2.2 &  35 &  0 \\
 36 &  \model{cafferesnet101} &  76.2 {\footnotesize \textcolor{gray}{[75.8, 76.6]}} &  78.3 {\footnotesize \textcolor{gray}{[77.4, 79.1]}} &  -2.1 &  37 &  -1 \\
 37 &  \model{resnet50} &  76.1 {\footnotesize \textcolor{gray}{[75.8, 76.5]}} &  78.1 {\footnotesize \textcolor{gray}{[77.3, 78.9]}} &  -2.0 &  38 &  -1 \\
 38 &  \model{dpn68} &  75.9 {\footnotesize \textcolor{gray}{[75.5, 76.2]}} &  78.4 {\footnotesize \textcolor{gray}{[77.6, 79.2]}} &  -2.6 &  36 &  2 \\
 39 &  \model{densenet169} &  75.6 {\footnotesize \textcolor{gray}{[75.2, 76.0]}} &  78.0 {\footnotesize \textcolor{gray}{[77.2, 78.8]}} &  -2.4 &  39 &  0 \\
 40 &  \model{resnet\_v2\_50\_tf} &  75.6 {\footnotesize \textcolor{gray}{[75.2, 76.0]}} &  78.0 {\footnotesize \textcolor{gray}{[77.2, 78.8]}} &  -2.4 &  40 &  0 \\
 41 &  \model{resnet\_v1\_50\_tf} &  75.2 {\footnotesize \textcolor{gray}{[74.8, 75.6]}} &  77.0 {\footnotesize \textcolor{gray}{[76.2, 77.9]}} &  -1.8 &  41 &  0 \\
 42 &  \model{densenet121} &  74.4 {\footnotesize \textcolor{gray}{[74.0, 74.8]}} &  76.8 {\footnotesize \textcolor{gray}{[75.9, 77.6]}} &  -2.3 &  45 &  -3 \\
 43 &  \model{vgg19\_bn} &  74.2 {\footnotesize \textcolor{gray}{[73.8, 74.6]}} &  76.6 {\footnotesize \textcolor{gray}{[75.7, 77.4]}} &  -2.3 &  46 &  -3 \\
 44 &  \model{pnasnet\_mobile\_tf} &  74.1 {\footnotesize \textcolor{gray}{[73.8, 74.5]}} &  76.8 {\footnotesize \textcolor{gray}{[76.0, 77.6]}} &  -2.7 &  44 &  0 \\
 45 &  \model{nasnetamobile} &  74.1 {\footnotesize \textcolor{gray}{[73.7, 74.5]}} &  76.4 {\footnotesize \textcolor{gray}{[75.5, 77.2]}} &  -2.3 &  47 &  -2 \\
 46 &  \model{inception\_v2\_tf} &  74.0 {\footnotesize \textcolor{gray}{[73.6, 74.4]}} &  77.0 {\footnotesize \textcolor{gray}{[76.1, 77.8]}} &  -3.0 &  43 &  3 \\
 47 &  \model{nasnet\_mobile\_tf} &  74.0 {\footnotesize \textcolor{gray}{[73.6, 74.4]}} &  76.0 {\footnotesize \textcolor{gray}{[75.1, 76.8]}} &  -2.0 &  49 &  -2 \\
 48 &  \model{bninception} &  73.5 {\footnotesize \textcolor{gray}{[73.1, 73.9]}} &  77.0 {\footnotesize \textcolor{gray}{[76.1, 77.8]}} &  -3.4 &  42 &  6 \\
 49 &  \model{vgg16\_bn} &  73.4 {\footnotesize \textcolor{gray}{[73.0, 73.7]}} &  75.9 {\footnotesize \textcolor{gray}{[75.1, 76.8]}} &  -2.6 &  50 &  -1 \\
 50 &  \model{resnet34} &  73.3 {\footnotesize \textcolor{gray}{[72.9, 73.7]}} &  76.3 {\footnotesize \textcolor{gray}{[75.4, 77.1]}} &  -3.0 &  48 &  2 \\
 51 &  \model{vgg19} &  72.4 {\footnotesize \textcolor{gray}{[72.0, 72.8]}} &  74.2 {\footnotesize \textcolor{gray}{[73.3, 75.0]}} &  -1.8 &  51 &  0 \\
 52 &  \model{vgg16} &  71.6 {\footnotesize \textcolor{gray}{[71.2, 72.0]}} &  73.9 {\footnotesize \textcolor{gray}{[73.0, 74.7]}} &  -2.3 &  52 &  0 \\
 53 &  \model{vgg13\_bn} &  71.6 {\footnotesize \textcolor{gray}{[71.2, 72.0]}} &  73.5 {\footnotesize \textcolor{gray}{[72.7, 74.4]}} &  -1.9 &  55 &  -2 \\
 54 &  \model{mobilenet\_v1\_tf} &  71.0 {\footnotesize \textcolor{gray}{[70.6, 71.4]}} &  72.4 {\footnotesize \textcolor{gray}{[71.5, 73.3]}} &  -1.4 &  59 &  -5 \\
 55 &  \model{vgg\_19\_tf} &  71.0 {\footnotesize \textcolor{gray}{[70.6, 71.4]}} &  73.6 {\footnotesize \textcolor{gray}{[72.7, 74.5]}} &  -2.6 &  53 &  2 \\
 56 &  \model{vgg\_16\_tf} &  70.9 {\footnotesize \textcolor{gray}{[70.5, 71.3]}} &  73.5 {\footnotesize \textcolor{gray}{[72.7, 74.4]}} &  -2.6 &  54 &  2 \\
 57 &  \model{vgg11\_bn} &  70.4 {\footnotesize \textcolor{gray}{[70.0, 70.8]}} &  73.0 {\footnotesize \textcolor{gray}{[72.1, 73.8]}} &  -2.6 &  58 &  -1 \\
 58 &  \model{vgg13} &  69.9 {\footnotesize \textcolor{gray}{[69.5, 70.3]}} &  72.0 {\footnotesize \textcolor{gray}{[71.1, 72.9]}} &  -2.1 &  60 &  -2 \\
 59 &  \model{inception\_v1\_tf} &  69.8 {\footnotesize \textcolor{gray}{[69.4, 70.2]}} &  73.1 {\footnotesize \textcolor{gray}{[72.2, 73.9]}} &  -3.3 &  56 &  3 \\
 60 &  \model{resnet18} &  69.8 {\footnotesize \textcolor{gray}{[69.4, 70.2]}} &  73.0 {\footnotesize \textcolor{gray}{[72.2, 73.9]}} &  -3.3 &  57 &  3 \\
 61 &  \model{vgg11} &  69.0 {\footnotesize \textcolor{gray}{[68.6, 69.4]}} &  70.8 {\footnotesize \textcolor{gray}{[69.9, 71.7]}} &  -1.8 &  61 &  0 \\
 62 &  \model{squeezenet1\_1} &  58.2 {\footnotesize \textcolor{gray}{[57.7, 58.6]}} &  61.7 {\footnotesize \textcolor{gray}{[60.7, 62.6]}} &  -3.5 &  62 &  0 \\
 63 &  \model{squeezenet1\_0} &  58.1 {\footnotesize \textcolor{gray}{[57.7, 58.5]}} &  60.7 {\footnotesize \textcolor{gray}{[59.7, 61.7]}} &  -2.6 &  63 &  0 \\
 64 &  \model{alexnet} &  56.5 {\footnotesize \textcolor{gray}{[56.1, 57.0]}} &  58.2 {\footnotesize \textcolor{gray}{[57.2, 59.1]}} &  -1.7 &  64 &  0 \\
 65 &  \model{fv\_64k} &  35.1 {\footnotesize \textcolor{gray}{[34.7, 35.5]}} &  34.2 {\footnotesize \textcolor{gray}{[33.3, 35.2]}} &  0.8 &  65 &  0 \\
 66 &  \model{fv\_16k} &  28.3 {\footnotesize \textcolor{gray}{[27.9, 28.7]}} &  27.4 {\footnotesize \textcolor{gray}{[26.6, 28.3]}} &  0.9 &  66 &  0 \\
 67 &  \model{fv\_4k} &  21.2 {\footnotesize \textcolor{gray}{[20.8, 21.5]}} &  21.1 {\footnotesize \textcolor{gray}{[20.3, 21.9]}} &  0.1 &  67 &  0 \\
\bottomrule
\end{tabular}


==> tables/imagenetv2-c-12_top5_model_results_table.tex <==
\begin{tabular}{rp{4.75cm}rrrrr}
\toprule 
\multicolumn{7}{c}{\textbf{ImageNet Top-5 \datasetc}} \\ 
\midrule
\multicolumn{1}{l}{Orig.} &                               &                                        &                                          &    & \multicolumn{1}{l}{New} &  \\ 
 \multicolumn{1}{l}{Rank} & Model & Orig. Accuracy & New Accuracy & Gap & \multicolumn{1}{l}{Rank} & $\Delta$ Rank \\
\midrule
 1 &  \model{pnasnet\_large\_tf} &  96.2 {\footnotesize \textcolor{gray}{[96.0, 96.3]}} &  97.2 {\footnotesize \textcolor{gray}{[96.9, 97.5]}} &  -1.0 &  2 &  -1 \\
 2 &  \model{nasnet\_large\_tf} &  96.2 {\footnotesize \textcolor{gray}{[96.0, 96.3]}} &  97.2 {\footnotesize \textcolor{gray}{[96.9, 97.5]}} &  -1.0 &  1 &  1 \\
 3 &  \model{nasnetalarge} &  96.0 {\footnotesize \textcolor{gray}{[95.8, 96.2]}} &  97.1 {\footnotesize \textcolor{gray}{[96.7, 97.4]}} &  -1.1 &  3 &  0 \\
 4 &  \model{pnasnet5large} &  96.0 {\footnotesize \textcolor{gray}{[95.8, 96.2]}} &  96.9 {\footnotesize \textcolor{gray}{[96.6, 97.2]}} &  -0.9 &  4 &  0 \\
 5 &  \model{polynet} &  95.6 {\footnotesize \textcolor{gray}{[95.4, 95.7]}} &  96.8 {\footnotesize \textcolor{gray}{[96.4, 97.1]}} &  -1.2 &  5 &  0 \\
 6 &  \model{senet154} &  95.5 {\footnotesize \textcolor{gray}{[95.3, 95.7]}} &  96.6 {\footnotesize \textcolor{gray}{[96.2, 97.0]}} &  -1.1 &  8 &  -2 \\
 7 &  \model{inception\_resnet\_v2\_tf} &  95.2 {\footnotesize \textcolor{gray}{[95.1, 95.4]}} &  96.8 {\footnotesize \textcolor{gray}{[96.4, 97.1]}} &  -1.5 &  6 &  1 \\
 8 &  \model{inception\_v4\_tf} &  95.2 {\footnotesize \textcolor{gray}{[95.0, 95.4]}} &  96.5 {\footnotesize \textcolor{gray}{[96.1, 96.9]}} &  -1.3 &  9 &  -1 \\
 9 &  \model{inceptionresnetv2} &  95.1 {\footnotesize \textcolor{gray}{[94.9, 95.3]}} &  96.7 {\footnotesize \textcolor{gray}{[96.3, 97.0]}} &  -1.5 &  7 &  2 \\
 10 &  \model{se\_resnext101\_32x4d} &  95.0 {\footnotesize \textcolor{gray}{[94.8, 95.2]}} &  96.2 {\footnotesize \textcolor{gray}{[95.8, 96.6]}} &  -1.2 &  11 &  -1 \\
 11 &  \model{inceptionv4} &  94.9 {\footnotesize \textcolor{gray}{[94.7, 95.1]}} &  96.4 {\footnotesize \textcolor{gray}{[96.0, 96.7]}} &  -1.5 &  10 &  1 \\
 12 &  \model{dpn107} &  94.7 {\footnotesize \textcolor{gray}{[94.5, 94.9]}} &  96.0 {\footnotesize \textcolor{gray}{[95.6, 96.4]}} &  -1.4 &  13 &  -1 \\
 13 &  \model{dpn92} &  94.6 {\footnotesize \textcolor{gray}{[94.4, 94.8]}} &  95.9 {\footnotesize \textcolor{gray}{[95.5, 96.3]}} &  -1.3 &  17 &  -4 \\
 14 &  \model{dpn131} &  94.6 {\footnotesize \textcolor{gray}{[94.4, 94.8]}} &  96.0 {\footnotesize \textcolor{gray}{[95.6, 96.4]}} &  -1.5 &  14 &  0 \\
 15 &  \model{dpn98} &  94.5 {\footnotesize \textcolor{gray}{[94.3, 94.7]}} &  96.0 {\footnotesize \textcolor{gray}{[95.6, 96.4]}} &  -1.5 &  15 &  0 \\
 16 &  \model{se\_resnext50\_32x4d} &  94.4 {\footnotesize \textcolor{gray}{[94.2, 94.6]}} &  95.9 {\footnotesize \textcolor{gray}{[95.5, 96.3]}} &  -1.5 &  18 &  -2 \\
 17 &  \model{se\_resnet152} &  94.4 {\footnotesize \textcolor{gray}{[94.2, 94.6]}} &  95.9 {\footnotesize \textcolor{gray}{[95.5, 96.3]}} &  -1.5 &  19 &  -2 \\
 18 &  \model{xception} &  94.3 {\footnotesize \textcolor{gray}{[94.1, 94.5]}} &  95.9 {\footnotesize \textcolor{gray}{[95.5, 96.3]}} &  -1.6 &  20 &  -2 \\
 19 &  \model{se\_resnet101} &  94.3 {\footnotesize \textcolor{gray}{[94.1, 94.5]}} &  95.9 {\footnotesize \textcolor{gray}{[95.5, 96.3]}} &  -1.6 &  21 &  -2 \\
 20 &  \model{resnext101\_64x4d} &  94.3 {\footnotesize \textcolor{gray}{[94.0, 94.5]}} &  95.7 {\footnotesize \textcolor{gray}{[95.3, 96.1]}} &  -1.5 &  23 &  -3 \\
 21 &  \model{resnet\_v2\_152\_tf} &  94.1 {\footnotesize \textcolor{gray}{[93.9, 94.3]}} &  96.0 {\footnotesize \textcolor{gray}{[95.6, 96.3]}} &  -1.9 &  16 &  5 \\
 22 &  \model{resnet152} &  94.0 {\footnotesize \textcolor{gray}{[93.8, 94.3]}} &  96.2 {\footnotesize \textcolor{gray}{[95.8, 96.5]}} &  -2.1 &  12 &  10 \\
 23 &  \model{inception\_v3\_tf} &  93.9 {\footnotesize \textcolor{gray}{[93.7, 94.1]}} &  95.5 {\footnotesize \textcolor{gray}{[95.1, 95.9]}} &  -1.5 &  25 &  -2 \\
 24 &  \model{resnext101\_32x4d} &  93.9 {\footnotesize \textcolor{gray}{[93.7, 94.1]}} &  95.2 {\footnotesize \textcolor{gray}{[94.8, 95.6]}} &  -1.3 &  31 &  -7 \\
 25 &  \model{se\_resnet50} &  93.8 {\footnotesize \textcolor{gray}{[93.5, 94.0]}} &  95.5 {\footnotesize \textcolor{gray}{[95.1, 95.9]}} &  -1.8 &  24 &  1 \\
 26 &  \model{resnet\_v2\_101\_tf} &  93.7 {\footnotesize \textcolor{gray}{[93.5, 93.9]}} &  95.8 {\footnotesize \textcolor{gray}{[95.4, 96.2]}} &  -2.1 &  22 &  4 \\
 27 &  \model{fbresnet152} &  93.6 {\footnotesize \textcolor{gray}{[93.4, 93.8]}} &  95.2 {\footnotesize \textcolor{gray}{[94.8, 95.7]}} &  -1.7 &  28 &  -1 \\
 28 &  \model{dpn68b} &  93.6 {\footnotesize \textcolor{gray}{[93.4, 93.8]}} &  95.2 {\footnotesize \textcolor{gray}{[94.8, 95.6]}} &  -1.6 &  32 &  -4 \\
 29 &  \model{densenet161} &  93.6 {\footnotesize \textcolor{gray}{[93.3, 93.8]}} &  95.2 {\footnotesize \textcolor{gray}{[94.8, 95.6]}} &  -1.7 &  29 &  0 \\
 30 &  \model{resnet101} &  93.5 {\footnotesize \textcolor{gray}{[93.3, 93.8]}} &  95.4 {\footnotesize \textcolor{gray}{[95.0, 95.8]}} &  -1.9 &  26 &  4 \\
 31 &  \model{inception\_v3} &  93.5 {\footnotesize \textcolor{gray}{[93.3, 93.7]}} &  95.1 {\footnotesize \textcolor{gray}{[94.7, 95.5]}} &  -1.6 &  34 &  -3 \\
 32 &  \model{inceptionv3} &  93.4 {\footnotesize \textcolor{gray}{[93.2, 93.6]}} &  95.2 {\footnotesize \textcolor{gray}{[94.8, 95.6]}} &  -1.8 &  30 &  2 \\
 33 &  \model{densenet201} &  93.4 {\footnotesize \textcolor{gray}{[93.1, 93.6]}} &  95.2 {\footnotesize \textcolor{gray}{[94.8, 95.7]}} &  -1.9 &  27 &  6 \\
 34 &  \model{resnet\_v1\_152\_tf} &  93.2 {\footnotesize \textcolor{gray}{[92.9, 93.4]}} &  95.2 {\footnotesize \textcolor{gray}{[94.7, 95.6]}} &  -2.0 &  33 &  1 \\
 35 &  \model{resnet\_v1\_101\_tf} &  92.9 {\footnotesize \textcolor{gray}{[92.7, 93.1]}} &  94.9 {\footnotesize \textcolor{gray}{[94.4, 95.3]}} &  -2.0 &  35 &  0 \\
 36 &  \model{resnet50} &  92.9 {\footnotesize \textcolor{gray}{[92.6, 93.1]}} &  94.7 {\footnotesize \textcolor{gray}{[94.2, 95.1]}} &  -1.8 &  39 &  -3 \\
 37 &  \model{resnet\_v2\_50\_tf} &  92.8 {\footnotesize \textcolor{gray}{[92.6, 93.1]}} &  94.8 {\footnotesize \textcolor{gray}{[94.3, 95.2]}} &  -1.9 &  37 &  0 \\
 38 &  \model{densenet169} &  92.8 {\footnotesize \textcolor{gray}{[92.6, 93.0]}} &  94.7 {\footnotesize \textcolor{gray}{[94.2, 95.1]}} &  -1.9 &  38 &  0 \\
 39 &  \model{dpn68} &  92.8 {\footnotesize \textcolor{gray}{[92.5, 93.0]}} &  94.8 {\footnotesize \textcolor{gray}{[94.3, 95.2]}} &  -2.0 &  36 &  3 \\
 40 &  \model{cafferesnet101} &  92.8 {\footnotesize \textcolor{gray}{[92.5, 93.0]}} &  94.6 {\footnotesize \textcolor{gray}{[94.1, 95.0]}} &  -1.8 &  40 &  0 \\
 41 &  \model{resnet\_v1\_50\_tf} &  92.2 {\footnotesize \textcolor{gray}{[92.0, 92.4]}} &  94.2 {\footnotesize \textcolor{gray}{[93.8, 94.7]}} &  -2.1 &  41 &  0 \\
 42 &  \model{densenet121} &  92.0 {\footnotesize \textcolor{gray}{[91.7, 92.2]}} &  94.0 {\footnotesize \textcolor{gray}{[93.5, 94.5]}} &  -2.0 &  46 &  -4 \\
 43 &  \model{pnasnet\_mobile\_tf} &  91.9 {\footnotesize \textcolor{gray}{[91.6, 92.1]}} &  94.1 {\footnotesize \textcolor{gray}{[93.6, 94.5]}} &  -2.2 &  44 &  -1 \\
 44 &  \model{vgg19\_bn} &  91.8 {\footnotesize \textcolor{gray}{[91.6, 92.1]}} &  94.0 {\footnotesize \textcolor{gray}{[93.5, 94.4]}} &  -2.1 &  47 &  -3 \\
 45 &  \model{inception\_v2\_tf} &  91.8 {\footnotesize \textcolor{gray}{[91.5, 92.0]}} &  94.2 {\footnotesize \textcolor{gray}{[93.7, 94.7]}} &  -2.5 &  42 &  3 \\
 46 &  \model{nasnetamobile} &  91.7 {\footnotesize \textcolor{gray}{[91.5, 92.0]}} &  94.1 {\footnotesize \textcolor{gray}{[93.6, 94.5]}} &  -2.3 &  43 &  3 \\
 47 &  \model{nasnet\_mobile\_tf} &  91.6 {\footnotesize \textcolor{gray}{[91.3, 91.8]}} &  93.8 {\footnotesize \textcolor{gray}{[93.4, 94.3]}} &  -2.3 &  49 &  -2 \\
 48 &  \model{bninception} &  91.6 {\footnotesize \textcolor{gray}{[91.3, 91.8]}} &  94.0 {\footnotesize \textcolor{gray}{[93.6, 94.5]}} &  -2.5 &  45 &  3 \\
 49 &  \model{vgg16\_bn} &  91.5 {\footnotesize \textcolor{gray}{[91.3, 91.8]}} &  93.7 {\footnotesize \textcolor{gray}{[93.2, 94.1]}} &  -2.1 &  50 &  -1 \\
 50 &  \model{resnet34} &  91.4 {\footnotesize \textcolor{gray}{[91.2, 91.7]}} &  93.9 {\footnotesize \textcolor{gray}{[93.4, 94.3]}} &  -2.5 &  48 &  2 \\
 51 &  \model{vgg19} &  90.9 {\footnotesize \textcolor{gray}{[90.6, 91.1]}} &  92.8 {\footnotesize \textcolor{gray}{[92.2, 93.3]}} &  -1.9 &  51 &  0 \\
 52 &  \model{vgg16} &  90.4 {\footnotesize \textcolor{gray}{[90.1, 90.6]}} &  92.5 {\footnotesize \textcolor{gray}{[92.0, 93.0]}} &  -2.1 &  53 &  -1 \\
 53 &  \model{vgg13\_bn} &  90.4 {\footnotesize \textcolor{gray}{[90.1, 90.6]}} &  92.6 {\footnotesize \textcolor{gray}{[92.1, 93.1]}} &  -2.2 &  52 &  1 \\
 54 &  \model{mobilenet\_v1\_tf} &  90.0 {\footnotesize \textcolor{gray}{[89.7, 90.2]}} &  91.4 {\footnotesize \textcolor{gray}{[90.8, 91.9]}} &  -1.4 &  59 &  -5 \\
 56 &  \model{vgg\_19\_tf} &  89.8 {\footnotesize \textcolor{gray}{[89.6, 90.1]}} &  92.1 {\footnotesize \textcolor{gray}{[91.5, 92.6]}} &  -2.2 &  56 &  0 \\
 55 &  \model{vgg\_16\_tf} &  89.8 {\footnotesize \textcolor{gray}{[89.6, 90.1]}} &  92.2 {\footnotesize \textcolor{gray}{[91.6, 92.7]}} &  -2.3 &  54 &  1 \\
 57 &  \model{vgg11\_bn} &  89.8 {\footnotesize \textcolor{gray}{[89.5, 90.1]}} &  91.9 {\footnotesize \textcolor{gray}{[91.4, 92.5]}} &  -2.1 &  58 &  -1 \\
 58 &  \model{inception\_v1\_tf} &  89.6 {\footnotesize \textcolor{gray}{[89.4, 89.9]}} &  92.1 {\footnotesize \textcolor{gray}{[91.6, 92.6]}} &  -2.5 &  55 &  3 \\
 59 &  \model{vgg13} &  89.2 {\footnotesize \textcolor{gray}{[89.0, 89.5]}} &  91.4 {\footnotesize \textcolor{gray}{[90.8, 91.9]}} &  -2.2 &  60 &  -1 \\
 60 &  \model{resnet18} &  89.1 {\footnotesize \textcolor{gray}{[88.8, 89.3]}} &  92.0 {\footnotesize \textcolor{gray}{[91.4, 92.5]}} &  -2.9 &  57 &  3 \\
 61 &  \model{vgg11} &  88.6 {\footnotesize \textcolor{gray}{[88.3, 88.9]}} &  91.0 {\footnotesize \textcolor{gray}{[90.4, 91.5]}} &  -2.4 &  61 &  0 \\
 62 &  \model{squeezenet1\_1} &  80.6 {\footnotesize \textcolor{gray}{[80.3, 81.0]}} &  83.9 {\footnotesize \textcolor{gray}{[83.1, 84.6]}} &  -3.2 &  62 &  0 \\
 63 &  \model{squeezenet1\_0} &  80.4 {\footnotesize \textcolor{gray}{[80.1, 80.8]}} &  83.5 {\footnotesize \textcolor{gray}{[82.8, 84.3]}} &  -3.1 &  63 &  0 \\
 64 &  \model{alexnet} &  79.1 {\footnotesize \textcolor{gray}{[78.7, 79.4]}} &  81.8 {\footnotesize \textcolor{gray}{[81.0, 82.6]}} &  -2.7 &  64 &  0 \\
 65 &  \model{fv\_64k} &  55.7 {\footnotesize \textcolor{gray}{[55.3, 56.2]}} &  55.9 {\footnotesize \textcolor{gray}{[54.9, 56.8]}} &  -0.1 &  65 &  0 \\
 66 &  \model{fv\_16k} &  49.9 {\footnotesize \textcolor{gray}{[49.5, 50.4]}} &  49.8 {\footnotesize \textcolor{gray}{[48.8, 50.8]}} &  0.1 &  66 &  0 \\
 67 &  \model{fv\_4k} &  41.3 {\footnotesize \textcolor{gray}{[40.8, 41.7]}} &  41.9 {\footnotesize \textcolor{gray}{[40.9, 42.8]}} &  -0.6 &  67 &  0 \\
\bottomrule
\end{tabular}


==> tables/subsampled_cifarv6_model_results_table.tex <==
\begin{tabular}{rp{4.75cm}rrrrr}
\toprule 
\multicolumn{7}{c}{\textbf{CIFAR-10}} \\ 
\midrule
\multicolumn{1}{l}{Orig.} &                                 &                                        &                                          &    & \multicolumn{1}{l}{New} &  \\ 
 \multicolumn{1}{l}{Rank} & Model & Orig. Accuracy & New Accuracy & Gap & \multicolumn{1}{l}{Rank} & $\Delta$ Rank \\
\midrule
 1 &  \model{autoaug\_pyramid\_net\_tf} &  98.4 {\footnotesize \textcolor{gray}{[98.1, 98.6]}} &  95.5 {\footnotesize \textcolor{gray}{[94.5, 96.4]}} &  2.9 &  1 &  0 \\
 6 &  \model{shake\_shake\_64d\_cutout} &  97.1 {\footnotesize \textcolor{gray}{[96.8, 97.4]}} &  93.1 {\footnotesize \textcolor{gray}{[91.9, 94.2]}} &  4.0 &  5 &  1 \\
 16 &  \model{wide\_resnet\_28\_10} &  95.9 {\footnotesize \textcolor{gray}{[95.5, 96.3]}} &  90.1 {\footnotesize \textcolor{gray}{[88.8, 91.4]}} &  5.8 &  13 &  3 \\
 23 &  \model{resnet\_basic\_110} &  93.5 {\footnotesize \textcolor{gray}{[93.0, 93.9]}} &  85.4 {\footnotesize \textcolor{gray}{[83.8, 86.9]}} &  8.1 &  24 &  -1 \\
 27 &  \model{vgg\_15\_BN\_64} &  93.0 {\footnotesize \textcolor{gray}{[92.5, 93.5]}} &  85.0 {\footnotesize \textcolor{gray}{[83.4, 86.6]}} &  7.9 &  27 &  0 \\
 30 &  \model{cudaconvnet} &  88.5 {\footnotesize \textcolor{gray}{[87.9, 89.2]}} &  78.2 {\footnotesize \textcolor{gray}{[76.3, 80.0]}} &  10.3 &  30 &  0 \\
 31 &  \model{random\_features\_256k\_aug} &  85.6 {\footnotesize \textcolor{gray}{[84.9, 86.3]}} &  73.6 {\footnotesize \textcolor{gray}{[71.6, 75.5]}} &  12.0 &  31 &  0 \\
\bottomrule
\end{tabular}

